Incomplete MaxSAT Approaches for Combinatorial Testing

We present a Satisfiability (SAT)-based approach for building Mixed Covering Arrays with Constraints of minimum length, referred to as the Covering Array Number problem. This problem is central in Combinatorial Testing for the detection of system failures. In particular, we show how to apply Maximum Satisfiability (MaxSAT) technology by describing efficient encodings for different classes of complete and incomplete MaxSAT solvers to compute optimal and suboptimal solutions, respectively. Similarly, we show how to solve through MaxSAT technology a closely related problem, the Tuple Number problem, which we extend to incorporate constraints. For this problem, we additionally provide a new MaxSAT-based incomplete algorithm. The extensive experimental evaluation we carry out on the available Mixed Covering Arrays with Constraints benchmarks and the comparison with state-of-the-art tools confirm the good performance of our approaches.

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/algo2_yamada.tex <==
\begin{algorithm}[ht]
    \SetAlgoRefName{CALOT}
    \caption{Algorithm 2 in \cite{YamadaKACOB15}}
    \label{alg:calot}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwInput}{Input:}
    \DontPrintSemicolon
    
    \KwInput{upper bound $ub$, strength $t$, SUT model $S$}
    
    $sat.add(Sat_{CCX}^{N=ub,t,S})$\;
    
    Fix $lb+1$ value tuples to break symmetries (see Section \ref{sec:symmetry})\;
    
    
    $b_{model} \leftarrow \emptyset$
    
    \For{$i=N,...,lb+1$} {
    
        \lIf{$sat.solve()=\mbox{UNSAT}$} {\Return{$(i, b_{model})$}}
        
        $sat.add(\bigwedge_{\tau \in \Tau} c^{i-1}_{\tau})$\;
        
        $b_{model} \leftarrow sat.model$\;
        
        \For{$\tau \in \Tau_a$}{
            \lFor{$(p,v) \in \tau$}{
                {$b_{model}[x_{i,p,v}]$
                \KwIfT $sat.add(\{x_{i,p,v}\})$ %
                \KwElseT $sat.add(\{\neg x_{i,p,v}\})$} %
            }
        }
    }
    \Return{$(lb+1, b_{model})$}\;
\end{algorithm}




==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/algo_forbidden.tex <==
\begin{algorithm}[ht]
    \SetAlgoRefName{ForbiddenTuples}
    \caption{Detection of forbidden tuples. \label{ForbiddenAlg}}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwInput}{Input:}
    \DontPrintSemicolon
    
    \KwInput{SUT model $S$, SAT solver $sat$}
    
    $sat.add(Sat_{CX}^{N=1,t,S}[\mbox{\ref{EqEOXs}}, \mbox{\ref{SUTX}}])$\;
    
    $\Tau_f = \emptyset$\;
    
    \For{$\tau \in \Tau$}{
        \For{$(p,v) \in \tau$}{
            $sat.assume(x_{1,p,v})$\;
        }
        \lIf{$sat.solve()=\mbox{UNSAT}$} {$\Tau_f \leftarrow \Tau_f \cup \tau$}
    }
    \Return{$\Tau_f$}
\end{algorithm}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/algo_hybrid.tex <==
\newcommand{\satcomm}[1]{\textsf{\scriptsize #1}}
\begin{algorithm}[h!t]
    \SetAlgoRefName{IncrementalCA}
    \caption{MaxSAT based Incremental Test Suite Construction \label{alg:hybridgreedy}}
    \SetKw{KwOr}{or}
    \SetKw{KwAnd}{and}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwGoTo}{go to}
    \SetKwProg{KwFunc}{function}{}{}
    \SetKw{KwInput}{Input:}
    \SetKwComment{KwComm}{\#}{}
    \DontPrintSemicolon
    
    \KwInput{SUT model $S$, Tests $N_i$ per iteration, SAT-based MaxSAT solver $msat$}

    
    $\Tau_r, \Upsilon \leftarrow \Tau_a, \emptyset$\;
    
    \While {$\Tau_r \neq \emptyset$ \KwAnd $|\Upsilon |<N$}{
        $N^\prime \leftarrow min(N_i, N-|\Upsilon |)$\;
    
        $msat.add\left ( TPMSat_{CCX}^{N^\prime,t,S} \right )$\;
    
        $msat.solve()$\; %
    
        $\upsilon \leftarrow \mbox{tests from } msat.model$\; 
        
        $\Upsilon \leftarrow \Upsilon \cup \upsilon$\;
        
        $\Tau_r \leftarrow \Tau_r \setminus \{\tau\ |\ \upsilon \models \tau\}$\;
    }
    \Return $\Upsilon $\;
\end{algorithm}
\let\satcomm\undefined

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/algo_incremental.tex <==
\newcommand{\satcomm}[1]{\textsf{\scriptsize #1}}
\begin{algorithm}[ht]
    \SetAlgoRefName{MSIncrementalCA}
    \caption{Incremental MaxSAT for Covering Array Construction \label{alg:incrmentalMS}}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwGoTo}{go to}
    \SetKwProg{KwFunc}{function}{}{}
    \SetKw{KwInput}{Input:}
    \SetKwComment{KwComm}{\#}{}
    \DontPrintSemicolon
    
    \KwInput{SUT model $S$, Tests $N_i$ per iteration, SAT-based MaxSAT solver $msat$}

    
    $T \leftarrow T \setminus ForbiddenTuples(S, msat)$ \KwComm{\satcomm{See Algorithm~\ref{ForbiddenAlg}}}
    
    $\phi_h, \phi_s \leftarrow PMSat_{CCX}^{N_i,t,S,lb}$
    
    $msat.add(\phi_h)$
    
    $msat.add\_retractable(\phi_s)$
    
    \While {$T \neq \emptyset$}{
    
    
        $msat.solve()$\; %
    
        $\gamma \leftarrow msat.model$\; 
        
        $\Gamma \leftarrow \Gamma \cup \gamma$\;
        
        Remove from $T$ the tuples covered by $\gamma$\;
        
        \hl{ TODO }
    }
\end{algorithm}
\let\satcomm\undefined

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/ex_ca_dummy_test.tex <==
   \begin{center}
    \begin{tabular}{@{\hskip 2mm}c@{\hskip 2mm}|@{\hskip 2mm}c@{\hskip 2mm}|@{\hskip 2mm}c@{\hskip 2mm}|@{\hskip 2mm}c@{\hskip 2mm}}
        \toprule
        L & E & S & M \\
        \midrule
        dy & ur & ra & cb \\
        \bottomrule
    \end{tabular} 
    \end{center}


==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/ex_ca_res_sat.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l|@{\hskip 2mm}c@{\hskip 2mm}|@{\hskip 2mm}c@{\hskip 2mm}|@{\hskip 2mm}c@{\hskip 2mm}|@{\hskip 2mm}c@{\hskip 2mm}}
        \toprule
         & L & E & S & M \\
        \midrule
        $t_1$ & dy & hw & ca & cb \\
        $t_2$ & ni & hw & ra & cb \\
        $t_3$ & ni & ur & ca & el \\
        $t_4$ & dy & ur & ra & cb \\
        $t_5$ & dy & ur & li & cb \\
        $t_6$ & dy & co & ca & cb \\
        $t_7$ & ni & co & ra & cb \\
        $t_8$ & dy & ur & ra & el \\
        $t_9$ & ni & ur & li & cb \\
        $t_{10}$ & ni & ur & li & el \\
        \bottomrule
    \end{tabular}
    \caption{$CA(10;2,S)$ for the autonomous driving SUT.}
    \label{tab:ex_ca_res_sat}
\end{table}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/ex_nux.tex <==
\begin{gather}
    \neg u_{10} \rightarrow (x_{10,L,dy} \wedge x_{10,E,ur} \wedge x_{10,S,ra} \wedge x_{10,M,cb}) \notag \\
    \neg u_{9} \rightarrow (x_{9,L,dy} \wedge x_{9,E,ur} \wedge x_{9,S,ra} \wedge x_{9,M,cb}) \tag{Ex. NUX} \\
    \neg u_{8} \rightarrow (x_{8,L,dy} \wedge x_{8,E,ur} \wedge x_{8,S,ra} \wedge x_{8,M,cb})\notag
\end{gather}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/pmsat_ccu.tex <==
\begin{gather}
    \neg c_{\tau_1}^{9} \rightarrow u_{10}, \quad \ldots, \quad \neg c_{\tau_{33}}^{9} \rightarrow u_{10} \notag \\
    \neg c_{\tau_1}^8 \rightarrow u_9, \quad \ldots, \quad \neg c_{\tau_{33}}^8 \rightarrow u_9 \tag{Ex. CCU} \\
    \neg c_{\tau_1}^7 \rightarrow u_8, \quad \ldots, \quad \neg c_{\tau_{33}}^7 \rightarrow u_8 \notag
\end{gather}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/pmsat_cu.tex <==
\begin{gather}
    c_{\tau_1}^{10} \rightarrow u_{10}, \quad \ldots, \quad c_{\tau_{33}}^{10} \rightarrow u_{10} \notag \\
    c_{\tau_1}^9 \rightarrow u_9, \quad \ldots, \quad c_{\tau_{33}}^9 \rightarrow u_9 \tag{Ex. CU} \\
    c_{\tau_1}^8 \rightarrow u_8, \quad \ldots, \quad c_{\tau_{33}}^8 \rightarrow u_8 \notag
\end{gather}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/pmsat_softu_bsu.tex <==

\begin{align}
\begin{gathered}
    (\neg u_{10}, 1) \notag \\
    (\neg u_9, 1) \tag{Ex. SoftU and BSU}  \\
    (\neg u_8, 1) \notag
\end{gathered}
&&
\begin{gathered}
    u_{10} \rightarrow u_9 \notag \\
    u_9 \rightarrow u_8 \notag
\end{gathered}
\end{align}


==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/pmsat_wsoftu.tex <==
\begin{gather}
    (\neg u_{10}, 3) \notag \\
    (\neg u_9, 2) \tag{Ex. WSoftU} \\
    (\neg u_8, 1) \notag
\end{gather}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sat_c.tex <==
\begin{equation}
    (c_{\tau_1}^1 \lor c_{\tau_1}^2 \lor \cdots \lor c_{\tau_1}^{10}), \quad \ldots, \quad (c_{\tau_{33}}^1 \lor c_{\tau_{33}}^2 \lor \cdots \lor c_{\tau_{33}}^{10}) \tag{Ex. C}
\end{equation}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sat_ccx.tex <==
\begin{gather}
    c_{\tau_1}^1 \rightarrow c_{\tau_1}^0 \lor x_{1,L,dy}, \quad \ldots, \quad c_{\tau_{33}}^1 \rightarrow c_{\tau_{33}}^0 \lor x_{1,M,el} \notag \\
    c_{\tau_1}^1 \rightarrow c_{\tau_1}^0 \lor x_{1,E,hw}, \quad \ldots, \quad c_{\tau_{33}}^1 \rightarrow c_{\tau_{33}}^0 \lor x_{1,S,li} \notag \\
    \vdots \qquad\qquad \ddots \qquad\qquad \vdots \tag{Ex. CCX a} \\
    c_{\tau_1}^{10} \rightarrow c_{\tau_1}^{9} \lor x_{10,L,dy}, \quad \ldots, \quad c_{\tau_{33}}^{10} \rightarrow c_{\tau_{33}}^9 \lor x_{10,M,el} \notag \\
    c_{\tau_1}^{10} \rightarrow c_{\tau_1}^{9} \lor x_{10,E,hw}, \quad \ldots, \quad c_{\tau_{33}}^{10} \rightarrow c_{\tau_{33}}^9 \lor x_{10,S,li} \notag \\
    c_{\tau_1}^{10}, \quad \ldots, \quad c_{\tau_{33}}^{10} \tag{Ex. CCX b} \\
    c_{\tau_1}^{10} \rightarrow \neg c_{\tau_1}^0, \quad \ldots, \quad c_{\tau_{33}}^{10} \rightarrow \neg c_{\tau_{33}}^0 \tag{Ex. CCX c}
\end{gather}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sat_cx.tex <==
\begin{gather}
    c_{\tau_1}^1 \rightarrow x_{1,L,dy}, \quad \ldots, \quad c_{\tau_{33}}^1 \rightarrow x_{1,M,el} \notag \\
    c_{\tau_1}^1 \rightarrow x_{1,E,hw}, \quad \ldots, \quad c_{\tau_{33}}^1 \rightarrow x_{1,S,li} \notag \\
    \vdots \qquad\qquad \ddots \qquad\qquad \vdots \tag{Ex. CX} \\
    c_{\tau_1}^{10} \rightarrow x_{10,L,dy}, \quad \ldots, \quad c_{\tau_{33}}^{10} \rightarrow x_{10,M,el} \notag \\
    c_{\tau_1}^{10} \rightarrow x_{10,E,hw}, \quad \ldots, \quad c_{\tau_{33}}^{10} \rightarrow x_{10,S,li} \notag
\end{gather}



==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sat_sutx.tex <==
\begin{gather}
(x_{1,L,ni} \land x_{1,E,co}) \rightarrow \neg x_{1,S,ca} \notag \\
(x_{1,E,hw} \lor x_{1,E,co}) \rightarrow \neg x_{1,S,li} \notag \\
x_{1,M,el} \rightarrow x_{1,E,ur} \notag \\
\vdots \tag{Ex. SUTX} \\
(x_{10,L,ni} \land x_{10,E,co}) \rightarrow \neg x_{10,S,ca} \notag \\
(x_{10,E,hw} \lor x_{10,E,co}) \rightarrow \neg x_{10,S,li} \notag \\
x_{10,M,el} \rightarrow x_{10,E,ur} \notag
\end{gather}



==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sat_x.tex <==
\begin{align}
   x_{1,L,dy} + x_{1,L,ni} =   &1,  & \mspace{-54.0mu} x_{1,E,hw} + x_{1,E,ur} + x_{1,E,co} =    &1, \notag\\
   x_{1,M,cb} + x_{1,M,el} =   &1,  & \mspace{-54.0mu} x_{1,S,ca} + x_{1,S,ra} + x_{1,S,li} =    &1{} \notag \\
                               &    & \mspace{-54.0mu}\vdots \hspace{3.8cm}                      &  \tag{Ex. X} \\
   x_{10,L,dy} + x_{10,L,ni} = &1,  & \mspace{-54.0mu} x_{10,E,hw} + x_{10,E,ur} + x_{10,E,co} = &1, \notag\\
   x_{10,M,cb} + x_{10,M,el} = &1,  & \mspace{-54.0mu} x_{10,S,ca} + x_{10,S,ra} + x_{10,S,li} = &1{} \notag 
\end{align}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sut.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{cc||c}
        \toprule
        $P \in S_P$ & Abbrv. & Values \\
        \midrule
        Luminosity & L & Day (dy), Night (ni) \\
        Environment & E & Highway (hw), Urban (ur), Country (co) \\
        Motor & M & Combustion (cb), Electric (el) \\
        Sensor & S & Camera (ca), Radar (ra), Lidar (li) \\
        \midrule
        \multicolumn{3}{c}{$S_\varphi$} \\ 
        \midrule
        \multicolumn{3}{c}{$((L = ni) \land (E = co)) \rightarrow (S \neq ca)$}\\
        \multicolumn{3}{c}{$((E = hw) \lor (E = co)) \rightarrow (S \neq li)$}\\
        \multicolumn{3}{c}{$(M = el) \rightarrow (E = ur)$} \\
        \bottomrule
    \end{tabular}
    \caption{Example of Autonomous Driving System Under Test.}
    \label{tab:sut}
\end{table}




==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/sym_x.tex <==
\begin{gather}
    x_{1,E,hw} \land x_{1,S,ca} \notag \\
    x_{2,E,hw} \land x_{2,S,ra} \notag \\
    x_{3,E,ur} \land x_{3,S,ca} \notag \\
    x_{4,E,ur} \land x_{4,S,ra} \tag{Ex. SYM X} \\
    x_{5,E,ur} \land x_{5,S,li} \notag \\
    x_{6,E,co} \land x_{6,S,ca} \notag \\
    x_{7,E,co} \land x_{7,S,ra} \notag
\end{gather}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/example/tn_rc_softc.tex <==
\begin{align}
\begin{gathered}
    c_{\tau_1} \leftrightarrow (c_{\tau_1}^1 \lor c_{\tau_1}^2 \lor \cdots \lor c_{\tau_1}^{10}) \notag \\
    \vdots \tag{Ex. RC and SoftC} \\
    c_{\tau_{33}} \leftrightarrow (c_{\tau_{33}}^1 \lor c_{\tau_{33}}^2 \lor \cdots \lor c_{\tau_{33}}^{10}) \notag
\end{gathered}
&&
\begin{gathered}
    (c_{\tau_1}, 1) \notag \\
    \vdots \notag \\
    (c_{\tau_{33}}, 1) \notag
\end{gathered}
\end{align}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/extra_functions.tex <==
\newcommand{\satcomm}[1]{\textsf{\scriptsize #1}}
\begin{algorithm}[h!t]%
    \SetAlgorithmName{Code}{SATSolver}{}
    \SetAlgoRefName{SATSolver}
    \caption{Members and functions interface}
    \label{alg:extra_funcs}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwInput}{Input:}
    \SetKw{KwAnd}{and}
    \SetKwProg{KwFunc}{function}{}{}
    \SetKwComment{KwComm}{\#}{}
    
    \SetKw{KwIff}{if}
    \SetKw{KwThenn}{then}
    \SetKw{KwElsee}{else}
    \DontPrintSemicolon
    
    \KwComm{\textbf{Attributes}}
    $n\_vars$ \KwComm{\satcomm{number of variables of the formula loaded}}
    $core$ \KwComm{\satcomm{last core found}}
    $model$ \KwComm{\satcomm{last model found}}
    
    \KwComm{\textbf{Methods}}
    
    \KwFunc{$assume(x : literal)$}{
       \KwComm{\satcomm{Sets the literal $x$ in the solver trail}}
    }
    \KwFunc{$add\_clause(c : clause)$}{
       \KwComm{\satcomm{Adds the clause $c$ to the solver}}
    }
    \KwFunc{$add\_retractable(c : clause)$}{
       \KwComm{\satcomm{Adds the clause $c$ to the retractable list of clauses of the solver}}
    }
    \KwFunc{$retract\_clause(c : clause)$}{
       \KwComm{\satcomm{Retracts the clause $c$ from the solver's list of retractable clauses}}
    }
    
    \KwFunc{$solve()$}{
        \KwComm{\satcomm{If formula is satisfiable, $status \leftarrow SAT, sat.model$ is updated}}
        \KwComm{\satcomm{If formula is unsatisfiable, $status \leftarrow UNSAT, sat.core$ is updated}}
        \KwRet{status}
    }
    
    \KwFunc {$add( \phi : \mbox{SAT formula} )$} {
        \lForEach{$c_i \in \phi$}{$sat.add\_clause(c_i)$}
    }
    \KwFunc {$retract(\phi  : \mbox{SAT formula} )$} {
        \lForEach{$c_i \in \phi$}{ $sat.retract\_clause(c_i)$}
    }
    
    \KwComm{\textbf{Overloaded functions for SAT-based MaxSAT algorithms}}
    
    \KwFunc {$add( \phi : \mbox{Weighted Partial MaxSAT formula} ) $} {
        \ForEach{$(c_i, w_i) \in \phi$}{
        \leIf{$w_i = \infty$}{$sat.add\_clause(c_i)$}{$sat.add\_retractable(c_i)$}
        }
    }
    \KwFunc {$retract(\phi  : \mbox{Weighted Partial MaxSAT formula})$} {
        \lForEach{$(c_i, w_i) \in \phi$}{
            \KwIff $w_i \neq \infty$ \KwThenn $sat.retract\_clause(c_i)$
        }
    }
\end{algorithm}
\let\satcomm\undefined

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/plots/plot_shortening_test_cmp.tex <==
\begin{figure}[h!t]
    \caption{Comparison of the required number of tests for different methods to cover as much tuples at each test from $\simeq T(N,t,S)$ (as base). %
    }
    \label{fig:hybrid-test-diff}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_1.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_11.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_20.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_spinv.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_NetworkMgmt.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_Storage5.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_RL-A-mod.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_RL-B-mod.pdf}
\end{figure}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/plots/plot_shortening_test_cmp_alt.tex <==
\begin{figure}[h!t]
    \caption{Comparison of the required number of tests for different methods to cover as much tuples at each test from $\simeq T(N,t,S)$ (as base). %
    }
    \label{fig:hybrid-test-diff}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_benchmark_1.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_benchmark_11.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_benchmark_20.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_benchmark_spinv.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_NetworkMgmt.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_Storage5.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_RL-A-mod.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tuples_Fig4/Gtuples_RL-B-mod.pdf}
\end{figure}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/plots/plot_shortening_tuple_cmp.tex <==
\begin{figure}[h!t]
    \caption{Comparison of the required number of tests for different methods with regards to the number of test used by $\simeq T(N,t,S)$ (as base) to cover each number of tuples. %
    }
    \label{fig:hybrid-tests}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_1.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_11.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_20.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_spinv.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_NetworkMgmt.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_Storage5.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_RL-A-mod.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_RL-B-mod.pdf}
\end{figure}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/plots/plot_shortening_tuple_cmp_alt.tex <==
\begin{figure}[h!t]
    \caption{Comparison of the required number of tests for different methods with regards to the number of test used by $\simeq T(N,t,S)$ (as base) to cover each number of tuples. %
    }
    \label{fig:hybrid-tests}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_benchmark_1.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_benchmark_11.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_benchmark_20.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_benchmark_spinv.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_NetworkMgmt.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_Storage5.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_RL-A-mod.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison_alt/tests_Fig3/Gtests_RL-B-mod.pdf}
\end{figure}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/plots/shoretning_loandra_sat4j_cmp.tex <==
\begin{figure}[h!t]
    \caption{Number of additional tuples covered by \emph{loandra} respect to \emph{linear} approach for different test suite sizes.}
    \label{fig:shortening-cmp}
    \centering
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_1.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_11.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_20.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_spinv.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/NetworkMgmt.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/Storage5.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/RL-A-mod.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/RL-B-mod.pdf}

\end{figure}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/plots/shortening_loandra.tex <==
\begin{figure}[h!t]
    \caption{Number of tests required to reach a certain coverage percentage for the \emph{tt-open-wbo-inc} approach.}
    \label{fig:shortening-tt-open-wbo-inc}
    \centering
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/benchmark_1.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/benchmark_11.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/benchmark_20.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/benchmark_spinv.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/NetworkMgmt.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/Storage5.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/RL-A-mod.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_tt-open-wbo-inc/RL-B-mod.pdf}

\end{figure}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/sat4j.tex <==
\begin{algorithm}[ht]
    \SetAlgoRefName{Linear}
    \caption{Linear SAT-based algorithm}
    \label{alg:linear}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwInput}{Input:}
    \DontPrintSemicolon
    
    
    \KwInput{Weighted Partial MaxSAT formula $\phi \equiv \phi_s \cup \phi_h$, SAT solver $sat$}
    
    $sat.add(\phi_h)$
    
    $sat.add(\{c_i \lor b_i | (c_i, w_i) \in \phi_s\})$
    
    $ub \leftarrow \sum_{(c_i,w_i) \in \phi_s} w_i + 1$
    
    $pb \leftarrow \sum_{(c_i,w_i) \in \phi_s} w_i \cdot b_i \leq ub-1$
    
    $sat.add(pb.to\_cnf)$
    
    \While{True} {
        \lIf{$sat.solve()=\mbox{UNSAT}$} {\Return{$(ub, sat.model)$}}
        
        $ub \leftarrow \sum_{(c_i,w_i) \in \phi_s} w_i \cdot sat.model[b_i]$
        
        $sat.add(pb.update(ub - 1))$
    }
    
\end{algorithm}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/table-maxsat-comp.tex <==
\begin{table}[h!]
\caption{COMPARISON WITH EXISTING SAT-BASED APPROACHES FOR 2-WAY COVERAGE}
\centering

\begin{tabular}{lll|cc|cc|cc|cc|cc}

\multicolumn{3}{c}{\textbf{}} & \multicolumn{2}{|c}{rc2-PM-2} & \multicolumn{2}{|c}{rc2-WPM-2} & \multicolumn{2}{|c}{algorithm2} & \multicolumn{2}{|c}{sat4j-PM-2} & \multicolumn{2}{|c}{sat4j-WPM-2} \\
Name & Model & Constraints & size & time & size & time & size & time & size & time & size & time \\
\midrule

1 & $2^{86}3^{3}4^{1}5^{5}6^{2}$ & $2^{20}3^{3}4^{1}$ & 48.00 & -1.00 & 38.00 & 3996.66 & 36.60* & 2652.88 & 36.50* & 2308.89 & 36.80* & \textbf{1649.59} \\ 

10 & $2^{130}3^{6}4^{5}5^{2}6^{4}$ & $2^{40}3^{7}$ & 47.00 & -1.00 & 43.00 & 4902.71 & \textbf{38.07} & 2443.95 & 38.10 & 2827.92 & 38.20 & 2162.16 \\ 

11 & $2^{84}3^{4}4^{2}5^{2}6^{4}$ & $2^{28}3^{4}$ & 47.00 & -1.00 & 41.00 & 3433.48 & 38.07 & 1855.12 & 38.00 & 1935.20 & \textbf{37.80} & 3169.15 \\ 

12 & $2^{136}3^{4}4^{3}5^{1}6^{3}$ & $2^{23}3^{4}$ & 36.00* & \textbf{43.63} & 36.00* & 44.33 & 36.00* & 121.76 & 36.00* & 178.08 & 36.00* & 158.01 \\ 

13 & $2^{124}3^{4}4^{1}5^{2}6^{2}$ & $2^{22}3^{4}$ & 36.00* & \textbf{24.47} & 36.00* & 25.02 & 36.00* & 81.66 & 36.00* & 79.84 & 36.00* & 28.48 \\ 

14 & $2^{81}3^{5}4^{3}6^{3}$ & $2^{13}3^{2}$ & 36.00* & \textbf{13.32} & 36.00* & 13.65 & 36.00* & 34.75 & 36.00* & 36.31 & 36.00* & 14.57 \\ 

15 & $2^{50}3^{4}4^{1}5^{2}6^{1}$ & $2^{20}3^{2}$ & 30.00* & 4.50 & 30.00* & 4.54 & 30.00* & 4.01 & 30.00* & 3.83 & 30.00* & \textbf{3.82} \\ 

16 & $2^{81}3^{3}4^{2}6^{1}$ & $2^{30}3^{4}$ & 24.00* & 6.09 & 24.00* & 6.05 & 24.00* & \textbf{5.55} & 24.00* & 5.78 & 24.00* & 5.77 \\ 

17 & $2^{128}3^{3}4^{2}5^{1}6^{3}$ & $2^{25}3^{4}$ & 36.00* & 30.30 & 36.00* & \textbf{29.76} & 36.00* & 110.03 & 36.00* & 109.52 & 36.00* & 115.03 \\ 

18 & $2^{127}3^{2}4^{4}5^{6}6^{2}$ & $2^{23}3^{4}4^{1}$ & 52.00 & -1.00 & 42.00 & 76.28 & 39.60 & 1674.05 & 39.50 & 3051.03 & \textbf{39.40} & 3579.32 \\ 

19 & $2^{172}3^{9}4^{9}5^{3}6^{4}$ & $2^{38}3^{5}$ & 51.00 & -1.00 & 46.00 & 109.47 & \textbf{40.47} & 3682.16 & 40.90 & 3627.69 & 40.60 & 2942.67 \\ 

2 & $2^{86}3^{3}4^{3}5^{1}6^{1}$ & $2^{19}3^{3}$ & 30.00* & 10.08 & 30.00* & 10.26 & 30.00* & 10.13 & 30.00* & 10.14 & 30.00* & \textbf{9.99} \\ 

20 & $2^{138}3^{4}4^{5}5^{4}6^{7}$ & $2^{42}3^{6}$ & 60.00 & -1.00 & 56.00 & 480.64 & 52.80 & 3412.95 & 52.70 & 3527.27 & \textbf{52.60} & 3134.99 \\ 

21 & $2^{76}3^{3}4^{2}5^{1}6^{3}$ & $2^{40}3^{6}$ & 36.00* & \textbf{9.89} & 36.00* & 10.06 & 36.00* & 10.17 & 36.00* & 10.63 & 36.00* & 10.37 \\ 

22 & $2^{72}3^{4}4^{1}6^{2}$ & $2^{20}3^{2}$ & 36.00* & 7.68 & 36.00* & 7.79 & 36.00* & 6.71 & 36.00* & \textbf{6.25} & 36.00* & 6.25 \\ 

23 & $2^{25}3^{1}6^{1}$ & $2^{13}3^{2}$ & 12.00* & 0.75 & 12.00* & 0.75 & 12.00* & 0.72 & 12.00* & 0.66 & 12.00* & \textbf{0.65} \\ 

24 & $2^{110}3^{2}5^{3}6^{4}$ & $2^{25}3^{4}$ & 48.00 & -1.00 & 44.00 & 448.46 & \textbf{40.13} & 1910.20 & 40.20 & 2058.91 & 40.20 & 2852.32 \\ 

25 & $2^{118}3^{6}4^{2}5^{2}6^{6}$ & $2^{23}3^{3}4^{1}$ & 52.00 & -1.00 & 52.00 & -1.00 & \textbf{47.33} & 3057.30 & 47.60 & 3032.79 & 47.80 & 2274.16 \\ 

26 & $2^{87}3^{1}4^{3}5^{4}$ & $2^{28}3^{4}$ & 34.00 & -1.00 & 27.00 & \textbf{110.50} & 26.00 & 328.98 & 26.00 & 281.25 & 26.00 & 210.68 \\ 

27 & $2^{55}3^{2}4^{2}5^{1}6^{2}$ & $2^{17}3^{3}$ & 36.00* & 5.56 & 36.00* & 5.64 & 36.00* & 4.35 & 36.00* & 4.33 & 36.00* & \textbf{4.30} \\ 

28 & $2^{167}3^{16}4^{2}5^{3}6^{6}$ & $2^{31}3^{6}$ & 57.00 & -1.00 & 53.00 & \textbf{304.47} & 48.60 & 4026.57 & 48.60 & 4637.53 & 48.60 & 4431.50 \\ 

29 & $2^{134}3^{7}5^{3}$ & $2^{19}3^{3}$ & 25.00* & \textbf{20.95} & 25.00* & 21.79 & 25.00* & 24.24 & 25.00* & 29.05 & 25.00* & 30.16 \\ 

3 & $2^{27}4^{2}$ & $2^{9}3^{1}$ & 17.58* & 0.92 & 18.00* & 0.92 & 18.00* & 0.87 & 18.00* & \textbf{0.79} & 18.00* & 0.80 \\ 

30 & $2^{73}3^{3}4^{3}$ & $2^{31}3^{4}$ & 16.00* & 4.98 & 16.00* & 5.32 & 16.00* & \textbf{4.88} & 16.00* & 5.22 & 16.00* & 5.30 \\ 

4 & $2^{51}3^{4}4^{2}5^{1}$ & $2^{15}3^{2}$ & 20.00* & 3.01 & 20.00* & 3.03 & 20.00* & \textbf{2.41} & 20.00* & 2.43 & 20.00* & 2.46 \\ 

5 & $2^{155}3^{7}4^{3}5^{5}6^{4}$ & $2^{32}3^{6}4^{1}$ & 54.00 & -1.00 & 47.00 & 385.93 & \textbf{44.67} & 3140.94 & 44.80 & 2719.70 & 44.80 & 2213.57 \\ 

6 & $2^{73}4^{3}6^{1}$ & $2^{26}3^{4}$ & 24.00* & 4.83 & 24.00* & 4.82 & 24.00* & 4.55 & 24.00* & \textbf{4.38} & 24.00* & 4.45 \\ 

7 & $2^{29}3^{1}$ & $2^{13}3^{2}$ & 12.00 & -1.00 & 9.00 & 1.35 & 9.00 & 1.34 & 9.00 & 1.09 & 9.00 & \textbf{1.08} \\ 

8 & $2^{109}3^{2}4^{2}5^{3}6^{3}$ & $2^{32}3^{4}4^{1}$ & 47.00 & -1.00 & 38.00 & \textbf{340.90} & 36.00* & 1347.87 & 36.00* & 1085.48 & 36.00* & 992.90 \\ 

9 & $2^{57}3^{1}4^{1}5^{1}6^{1}$ & $2^{30}3^{7}$ & 20.00* & 2.80 & 20.00* & 2.85 & 20.00* & \textbf{2.20} & 20.00* & 2.25 & 20.00* & 2.24 \\ 

apache & $2^{158}3^{8}4^{4}5^{1}6^{1}$ & $2^{3}3^{1}4^{2}5^{1}$ & 30.00* & \textbf{33.58} & 30.00* & 35.32 & 30.00* & 111.19 & 30.00* & 105.05 & 30.00* & 110.21 \\ 

bugzilla & $2^{49}3^{1}4^{2}$ & $2^{4}3^{1}$ & 16.00* & 2.10 & 16.00* & 2.14 & 16.00* & \textbf{1.97} & 16.00* & 2.04 & 16.00* & 2.02 \\ 

gcc & $2^{189}3^{10}$ & $2^{37}3^{3}$ & 23.00 & -1.00 & 15.00 & \textbf{39.49} & 15.00 & 158.53 & 15.00 & 225.79 & 15.00 & 259.00 \\ 

spins & $2^{13}4^{5}$ & $2^{13}$ & 18.00* & \textbf{0.86} & 19.00* & 0.94 & 19.00* & 1.06 & 19.00* & 0.93 & 19.00* & 1.65 \\ 

spinv & $2^{42}3^{2}4^{11}$ & $2^{47}3^{2}$ & 45.00 & -1.00 & 32.00 & 134.94 & 31.00 & 115.57 & 31.00 & 153.66 & 31.00 & \textbf{90.75} \\ 

\end{tabular}

\end{table}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/tables/inst_sizes.tex <==
\begin{table}[h!t]

\centering

\resizebox{\textwidth}{!}{

\begin{tabular}{l|llr|rcrrr|rrrr}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{3}{c|}{System Under Test (SUT)} & \multicolumn{5}{c|}{Bounds for $t = 2$} & \multicolumn{4}{c}{$PMSat_{CCX}^{N,t=2,S,lb}$} \\

Instance & $S_P$ & $S_{\varphi}$ & \makecell[bc]{\# lits \\ $CNF(S_{\varphi})$} & $ub^{ACTS}$ & $ub^{\simeq}$ & lb & $|\Tau_a|$ & $|\Tau_f|$ & \# vars & \# clauses & \# lits & size (MB) \\
\midrule

Cohen et al. \cite{cohen2008constructing} &  &  &  &  &  &  &  &  &  &  &  & \\

\midrule
1 & $2^{86}3^{3}4^{1}5^{5}6^{2}$ & $2^{20}3^{3}4^{1}$ & 53 & 48 & 37 & 35 & 23876 & 474 & 1158588 & 2620675 & 7463282 & 60.01 \\
2 & $2^{86}3^{3}4^{3}5^{1}6^{1}$ & $2^{19}3^{3}$ & 47 & 32 & 30* & 29 & 20331 & 237 & 657890 & 1371738 & 3984183 & 29.91 \\
3 & $2^{27}4^{2}$ & $2^{9}3^{1}$ & 21 & 19 & 18* & 15 & 1838 & 14 & 36217 & 79008 & 222390 & 1.47 \\
4 & $2^{51}3^{4}4^{2}5^{1}$ & $2^{15}3^{2}$ & 36 & 22 & 20* & 19 & 7530 & 386 & 168852 & 358291 & 1025536 & 7.33 \\
5 & $2^{155}3^{7}4^{3}5^{5}6^{4}$ & $2^{32}3^{6}4^{1}$ & 86 & 54 & 45 & 35 & 76259 & 73 & 4142574 & 9720622 & 27451121 & 236.74 \\
6 & $2^{73}4^{3}6^{1}$ & $2^{26}3^{4}$ & 64 & 25 & 24* & 23 & 11382 & 1878 & 289001 & 597814 & 1730859 & 12.72 \\
7 & $2^{29}3^{1}$ & $2^{13}3^{2}$ & 32 & 12 & 9 & 5 & 1567 & 231 & 19566 & 49758 & 132435 & 0.85 \\
8 & $2^{109}3^{2}4^{2}5^{3}6^{3}$ & $2^{32}3^{4}4^{1}$ & 80 & 47 & 36* & 35 & 33680 & 1098 & 1597165 & 3590459 & 10247230 & 84.50 \\
9 & $2^{57}3^{1}4^{1}5^{1}6^{1}$ & $2^{30}3^{7}$ & 81 & 22 & 20* & 19 & 6835 & 1720 & 153584 & 325984 & 932515 & 6.63 \\
10 & $2^{130}3^{6}4^{5}5^{2}6^{4}$ & $2^{40}3^{7}$ & 101 & 47 & 41 & 35 & 52659 & 2029 & 2493173 & 5608369 & 16010703 & 135.34 \\
11 & $2^{84}3^{4}4^{2}5^{2}6^{4}$ & $2^{28}3^{4}$ & 68 & 47 & 39 & 35 & 23636 & 707 & 1123311 & 2523897 & 7200149 & 57.70 \\
12 & $2^{136}3^{4}4^{3}5^{1}6^{3}$ & $2^{23}3^{4}$ & 58 & 43 & 36* & 35 & 49522 & 978 & 2144718 & 4675267 & 13461992 & 108.23 \\
13 & $2^{124}3^{4}4^{1}5^{2}6^{2}$ & $2^{22}3^{4}$ & 56 & 40 & 36* & 35 & 38862 & 1701 & 1567084 & 3319517 & 9632256 & 75.77 \\
14 & $2^{81}3^{5}4^{3}6^{3}$ & $2^{13}3^{2}$ & 32 & 39 & 36* & 35 & 20544 & 618 & 810618 & 1697204 & 4936072 & 37.18 \\
15 & $2^{50}3^{4}4^{1}5^{2}6^{1}$ & $2^{20}3^{2}$ & 46 & 32 & 30* & 29 & 8388 & 155 & 273410 & 569181 & 1650514 & 12.10 \\
16 & $2^{81}3^{3}4^{2}6^{1}$ & $2^{30}3^{4}$ & 72 & 25 & 24* & 23 & 14600 & 2303 & 370051 & 765960 & 2218422 & 16.44 \\
17 & $2^{128}3^{3}4^{2}5^{1}6^{3}$ & $2^{25}3^{4}$ & 62 & 41 & 36* & 35 & 43390 & 66 & 1792402 & 3835891 & 11100545 & 88.14 \\
18 & $2^{127}3^{2}4^{4}5^{6}6^{2}$ & $2^{23}3^{4}4^{1}$ & 62 & 52 & 41 & 35 & 50128 & 28 & 2625808 & 6092947 & 17250882 & 146.38 \\
19 & $2^{172}3^{9}4^{9}5^{3}6^{4}$ & $2^{38}3^{5}$ & 91 & 51 & 43 & 35 & 98778 & 114 & 5064366 & 11694341 & 33170488 & 287.31 \\
20 & $2^{138}3^{4}4^{5}5^{4}6^{7}$ & $2^{42}3^{6}$ & 102 & 60 & 54 & 35 & 64620 & 3320 & 3903864 & 9411047 & 26386102 & 227.62 \\
21 & $2^{76}3^{3}4^{2}5^{1}6^{3}$ & $2^{40}3^{6}$ & 98 & 39 & 36* & 35 & 15442 & 2742 & 610938 & 1279170 & 3717471 & 27.90 \\
22 & $2^{72}3^{4}4^{1}6^{2}$ & $2^{20}3^{2}$ & 46 & 37 & 36* & 35 & 13405 & 1181 & 503127 & 1028139 & 3008516 & 22.48 \\
23 & $2^{25}3^{1}6^{1}$ & $2^{13}3^{2}$ & 32 & 14 & 12* & 11 & 1495 & 173 & 21856 & 47740 & 132915 & 0.85 \\
24 & $2^{110}3^{2}5^{3}6^{4}$ & $2^{25}3^{4}$ & 62 & 48 & 41 & 35 & 34204 & 570 & 1656252 & 3748659 & 10679658 & 88.30 \\
25 & $2^{118}3^{6}4^{2}5^{2}6^{6}$ & $2^{23}3^{3}4^{1}$ & 59 & 52 & 49 & 35 & 46968 & 52 & 2461280 & 5710735 & 16167454 & 136.81 \\
26 & $2^{87}3^{1}4^{3}5^{4}$ & $2^{28}3^{4}$ & 68 & 34 & 26 & 24 & 20921 & 667 & 719347 & 1643461 & 4647485 & 36.52 \\
27 & $2^{55}3^{2}4^{2}5^{1}6^{2}$ & $2^{17}3^{3}$ & 43 & 37 & 36* & 35 & 9714 & 43 & 365524 & 746797 & 2183919 & 16.18 \\
28 & $2^{167}3^{16}4^{2}5^{3}6^{6}$ & $2^{31}3^{6}$ & 80 & 57 & 50 & 35 & 96599 & 74 & 5535861 & 13181074 & 37087871 & 322.33 \\
29 & $2^{134}3^{7}5^{3}$ & $2^{19}3^{3}$ & 47 & 29 & 25* & 24 & 45839 & 32 & 1338905 & 2899941 & 8321499 & 64.34 \\
30 & $2^{73}3^{3}4^{3}$ & $2^{31}3^{4}$ & 74 & 22 & 16* & 15 & 12453 & 1308 & 277976 & 640938 & 1792681 & 13.16 \\
apache & $2^{158}3^{8}4^{4}5^{1}6^{1}$ & $2^{3}3^{1}4^{2}5^{1}$ & 22 & 33 & 30* & 29 & 66927 & 3 & 2221926 & 4701044 & 13619419 & 109.16 \\
bugzilla & $2^{49}3^{1}4^{2}$ & $2^{4}3^{1}$ & 11 & 19 & 16* & 15 & 5818 & 4 & 112768 & 247130 & 697953 & 4.82 \\
gcc & $2^{189}3^{10}$ & $2^{37}3^{3}$ & 83 & 23 & 15 & 8 & 82770 & 39 & 1913568 & 5063264 & 13685896 & 112.78 \\
spins & $2^{13}4^{5}$ & $2^{13}$ & 26 & 26 & 19* & 15 & 979 & 13 & 27050 & 64498 & 177169 & 1.23 \\
spinv & $2^{42}3^{2}4^{11}$ & $2^{47}3^{2}$ & 100 & 45 & 33 & 15 & 8741 & 56 & 401069 & 1063265 & 2888090 & 22.53 \\
\midrule

Segall et al. \cite{segall11} &  &  &  &  &  &  &  &  &  &  &  & \\

\midrule
Banking1 & $3^{4}4^{1}$ & $5^{112}$ & 560 & 15 & 13* & 11 & 102 & 0 & 1938 & 5864 & 19573 & 0.11 \\
Banking2 & $2^{14}4^{1}$ & $2^{3}$ & 6 & 11 & 10* & 7 & 473 & 3 & 5591 & 12845 & 34672 & 0.21 \\
CommProtocol & $2^{10}7^{1}$ & \makecell[cl]{$2^{10}3^{10}4^{12}5^{24}$ \\ $6^{30}7^{30}8^{12}$} & 704 & 19 & 16* & 13 & 285 & 35 & 6047 & 15914 & 50363 & 0.29 \\
Concurrency & $2^{5}$ & $2^{4}3^{1}5^{2}$ & 21 & 6 & 5* & 3 & 36 & 4 & 278 & 667 & 1686 & 0.01 \\
Healthcare1 & $2^{6}3^{2}5^{1}6^{1}$ & $2^{3}3^{18}$ & 60 & 30 & 30* & 29 & 361 & 8 & 12090 & 24661 & 70619 & 0.44 \\
Healthcare2 & $2^{5}3^{6}4^{1}$ & $2^{1}3^{6}5^{18}$ & 110 & 16 & 14 & 11 & 466 & 1 & 8212 & 18853 & 52268 & 0.31 \\
Healthcare3 & $2^{16}3^{6}4^{5}5^{1}6^{1}$ & $2^{31}$ & 62 & 38 & 34* & 29 & 3092 & 59 & 121950 & 271023 & 768538 & 5.38 \\
Healthcare4 & $2^{13}3^{12}4^{6}5^{2}6^{1}7^{1}$ & $2^{22}$ & 44 & 49 & 46* & 41 & 5707 & 38 & 287980 & 619634 & 1783211 & 13.14 \\
Insurance & $2^{6}3^{1}5^{1}6^{2}11^{1}13^{1}17^{1}31^{1}$ & - & 0 & 527 & 527* & 526 & 4573 & 0 & 2509047 & 5009492 & 14863678 & 122.95 \\
NetworkMgmt & $2^{2}4^{1}5^{3}10^{2}11^{1}$ & $2^{20}$ & 40 & 112 & 110* & 109 & 1228 & 20 & 148402 & 301059 & 877206 & 6.28 \\
ProcessorComm1 & $2^{3}3^{6}4^{6}$ & $2^{13}$ & 26 & 29 & 21 & 15 & 1058 & 13 & 32957 & 80475 & 219601 & 1.54 \\
ProcessorComm2 & $2^{3}3^{12}4^{8}5^{2}$ & $1^{4}2^{121}$ & 246 & 32 & 25* & 24 & 2525 & 854 & 85287 & 193248 & 541399 & 3.73 \\
Services & $2^{3}3^{4}5^{2}8^{2}10^{2}$ & $3^{386}4^{2}$ & 1166 & 106 & 100* & 99 & 1819 & 16 & 204692 & 460866 & 1346965 & 9.78 \\
Storage1 & $2^{1}3^{1}4^{1}5^{1}$ & $4^{95}$ & 380 & 17 & 17* & 14 & 53 & 18 & 1294 & 4270 & 13468 & 0.07 \\
Storage2 & $3^{4}6^{1}$ & - & 0 & 18 & 18* & 17 & 126 & 0 & 2826 & 5652 & 15552 & 0.09 \\
Storage3 & $2^{9}3^{1}5^{3}6^{1}8^{1}$ & $2^{38}3^{10}$ & 106 & 50 & 50* & 39 & 1020 & 120 & 54810 & 122009 & 344328 & 2.47 \\
Storage4 & $2^{5}3^{7}4^{1}5^{2}6^{2}7^{1}10^{1}13^{1}$ & $2^{24}$ & 48 & 136 & 130* & 129 & 3491 & 24 & 495046 & 1012862 & 2970799 & 22.45 \\
Storage5 & $2^{5}3^{8}5^{3}6^{2}8^{1}9^{1}10^{2}11^{1}$ & $2^{151}$ & 302 & 218 & 215 & 109 & 5342 & 246 & 1206084 & 3020149 & 8366680 & 72.16 \\
SystemMgmt & $2^{5}3^{4}5^{1}$ & $2^{13}3^{4}$ & 38 & 17 & 15* & 14 & 310 & 14 & 5935 & 12813 & 35376 & 0.21 \\
Telecom & $2^{5}3^{1}4^{2}5^{1}6^{1}$ & $2^{11}3^{1}4^{9}$ & 61 & 32 & 30* & 29 & 440 & 11 & 15650 & 32761 & 93262 & 0.59 \\
\midrule

Yu et al. \cite{Yu15} &  &  &  &  &  &  &  &  &  &  &  & \\

\midrule
RL-A & $2^{5}3^{4}4^{7}5^{4}6^{5}7^{4}8^{1}12^{3}$ & $1^{12}2^{491}3^{345}$ & 2029 & 155 & 153 & 143 & 7066 & 7156 & 1142671 & 2491775 & 7220414 & 59.32 \\
RL-B & \makecell[cl]{$2^{8}3^{2}4^{3}5^{3}6^{1}9^{1}$ \\ $10^{1}12^{2}14^{3}20^{1}24^{1}37^{1}$} & \makecell[cl]{$1^{8}2^{1127}3^{277}$ \\ $4^{1755}5^{1064}6^{2048}$} & 27721 & 767 & 727 & 519 & 17018 & 5597 & 13365222 & 35733711 & 109278283 & 1026.60 \\
\midrule %

Yamada et al. \cite{Yamada16} &  &  &  &  &  &  &  &  &  &  &  & \\

\midrule
Company2 & $2^{6}3^{4}8^{4}$ & \makecell[cl]{$1^{2}2^{35}3^{89}4^{54}5^{34}$ \\ $6^{20}7^{34}8^{16}9^{4}$} & 1247 & 81 & 72 & 55 & 1149 & 261 & 100546 & 252543 & 744203 & 5.35 \\
\bottomrule
\end{tabular}

}
\caption{General information of all benchmarks used.}
\label{tab:inst-sizes}
\end{table}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/tables/table_ca.tex <==
\begin{table}[h!t]

\centering

\resizebox{0.83\textwidth}{!}{

\begin{tabular}{l|cr|cr|cr|cr|cr}
\toprule
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{CALOT} & \multicolumn{2}{c|}{RC2-PM} & \multicolumn{2}{c|}{RC2-WPM} & \multicolumn{2}{c|}{Linear-PM} & \multicolumn{2}{c}{Linear-WPM} \\
Instance & size & time & size & time & size & time & size & time & size & time \\
\midrule %

Cohen et al. \cite{cohen2008constructing} & & & & & & & & & & \\

\midrule

1 & 36.60* & 2097.94 & 38.40* & - & 36.40* & 2746.61 & 36.40* & 2666.12 & 36.40* & \textbf{1767.29} \\ 

2 & 30.00* & \textbf{9.63} & 30.00* & \textbf{12.05} & 30.00* & \textbf{12.72} & 30.00* & \textbf{10.44} & 30.00* & \textbf{10.54} \\ 

3 & 18.00* & \textbf{0.79} & 18.00* & \textbf{0.97} & 18.00* & \textbf{0.99} & 18.00* & \textbf{0.78} & 18.00* & \textbf{0.78} \\ 

4 & 20.00* & \textbf{2.27} & 20.00* & \textbf{3.13} & 20.00* & \textbf{3.22} & 20.00* & \textbf{2.38} & 20.00* & \textbf{2.35} \\ 

5 & 44.60 & 3039.80 & 54.00 & - & 44.60 & 3004.00 & 44.70 & 2538.28 & \textbf{44.40} & 3098.15 \\ 

6 & 24.00* & \textbf{4.33} & 24.00* & \textbf{5.56} & 24.00* & \textbf{5.50} & 24.00* & \textbf{5.02} & 24.00* & \textbf{4.98} \\ 

7 & 9.00 & \textbf{1.00} & 12.00 & - & 9.00 & \textbf{1.63} & 9.00 & \textbf{1.27} & 9.00 & \textbf{1.21} \\ 

8 & 36.00* & 1024.22 & 36.00* & 1019.61 & 36.00* & 1221.64 & 36.00* & 1227.26 & 36.00* & \textbf{944.89} \\ 

9 & 20.00* & \textbf{2.15} & 20.00* & \textbf{2.91} & 20.00* & \textbf{2.92} & 20.00* & \textbf{2.30} & 20.00* & \textbf{2.28} \\ 

10 & 38.30 & 1960.09 & 47.00 & - & 38.20 & 2322.41 & \textbf{38.10} & 2901.29 & 38.50 & 1962.17 \\ 

11 & 37.90 & 2701.45 & 47.00 & - & 37.90 & 2305.90 & 37.80 & 2808.34 & \textbf{37.70} & 2799.72 \\ 

12 & 36.00* & \textbf{114.89} & 36.00* & \textbf{118.78} & 36.00* & 194.74 & 36.00* & 148.69 & 36.00* & 143.26 \\ 

13 & 36.00* & 78.88 & 36.00* & \textbf{31.70} & 36.00* & 93.00 & 36.00* & \textbf{34.63} & 36.00* & \textbf{33.34} \\ 

14 & 36.00* & 32.78 & 36.00* & \textbf{14.68} & 36.00* & \textbf{17.00} & 36.00* & 34.61 & 36.00* & 36.91 \\ 

15 & 30.00* & \textbf{3.85} & 30.00* & \textbf{4.77} & 30.00* & \textbf{4.86} & 30.00* & \textbf{3.68} & 30.00* & \textbf{3.61} \\ 

16 & 24.00* & \textbf{5.27} & 24.00* & \textbf{7.58} & 24.00* & \textbf{7.61} & 24.00* & \textbf{5.78} & 24.00* & \textbf{5.71} \\ 

17 & 36.00* & 99.88 & 36.00* & \textbf{65.09} & 36.00* & 125.62 & 36.00* & 104.08 & 36.00* & 112.25 \\ 

18 & 39.70 & 1825.61 & 52.00 & - & 39.30 & \textbf{2112.41} & 39.40 & 3560.15 & 39.30 & 3794.11 \\ 

19 & 40.50 & 3494.11 & 51.00 & - & 40.60 & 3627.53 & 40.80 & 3356.22 & \textbf{40.40} & 4150.12 \\ 

20 & 52.70 & 3719.47 & 60.00 & - & \textbf{52.50} & \textbf{3571.71} & 52.90 & 3743.61 & 52.70 & 4096.86 \\ 

21 & 36.00* & \textbf{9.73} & 36.00* & \textbf{11.63} & 36.00* & \textbf{12.00} & 36.00* & \textbf{9.73} & 36.00* & \textbf{9.83} \\ 

22 & 36.00* & \textbf{6.32} & 36.00* & \textbf{9.03} & 36.00* & \textbf{9.17} & 36.00* & \textbf{7.00} & 36.00* & \textbf{6.94} \\ 

23 & 12.00* & \textbf{0.65} & 12.00* & \textbf{0.74} & 12.00* & \textbf{0.74} & 12.00* & \textbf{0.60} & 12.00* & \textbf{0.60} \\ 

24 & 40.10 & \textbf{2322.47} & 48.00 & - & 40.60 & 1434.60 & 40.10 & 3233.78 & 40.10 & 2373.92 \\ 

25 & 47.30 & 3502.14 & 52.00 & - & 47.50 & 3792.21 & \textbf{47.10} & 3295.66 & 47.30 & 3135.00 \\ 

26 & 26.00 & 251.66 & 34.00 & - & 26.00 & \textbf{165.95} & 26.00 & 187.65 & 26.00 & 254.04 \\ 

27 & 36.00* & \textbf{4.08} & 36.00* & \textbf{6.20} & 36.00* & \textbf{6.21} & 36.00* & \textbf{4.39} & 36.00* & \textbf{4.33} \\ 

28 & \textbf{48.40} & 4034.09 & 57.00 & - & 48.50 & 4436.71 & 48.50 & 4082.97 & 48.60 & 3904.62 \\ 

29 & 25.00* & \textbf{22.93} & 25.00* & 58.71 & 25.00* & 65.48 & 25.00* & 32.20 & 25.00* & 29.63 \\ 

30 & 16.00* & \textbf{4.59} & 16.00* & \textbf{5.71} & 16.00* & \textbf{6.22} & 16.00* & \textbf{6.04} & 16.00* & \textbf{6.05} \\ 

apache & 30.00* & 106.62 & 30.00* & \textbf{93.83} & 30.00* & 117.45 & 30.00* & 124.21 & 30.00* & 118.02 \\ 

bugzilla & 16.00* & \textbf{1.84} & 16.00* & \textbf{2.36} & 16.00* & \textbf{2.39} & 16.00* & \textbf{1.97} & 16.00* & \textbf{1.95} \\ 

gcc & 15.00 & \textbf{149.50} & 23.00 & - & 15.00 & 187.58 & 15.00 & 253.12 & 15.00 & 250.03 \\ 

spins & 19.00* & \textbf{0.96} & 19.00* & \textbf{1.00} & 19.00* & \textbf{1.69} & 19.00* & \textbf{1.41} & 19.00* & \textbf{1.38} \\ 

spinv & 31.00 & \textbf{106.02} & 45.00 & - & 31.00 & \textbf{104.61} & 31.00 & \textbf{110.06} & 31.00 & \textbf{106.76} \\ 

\midrule %

Segall et al. \cite{segall11} & & & & & & & & & & \\

\midrule

Banking1 & 13.00* & \textbf{0.57} & 13.00* & \textbf{0.45} & 13.00* & \textbf{0.51} & 13.00* & \textbf{0.45} & 13.00* & \textbf{0.40} \\ 

Banking2 & 10.00* & \textbf{9.04} & 10.00* & \textbf{14.47} & 10.00* & \textbf{14.38} & 10.00* & \textbf{9.25} & 10.00* & \textbf{9.11} \\ 

CommProtocol & 16.00* & \textbf{0.50} & 16.00* & \textbf{0.40} & 16.00* & \textbf{0.46} & 16.00* & \textbf{0.39} & 16.00* & \textbf{0.35} \\ 

Concurrency & 5.00* & \textbf{0.40} & 5.00* & \textbf{0.28} & 5.00* & \textbf{0.32} & 5.00* & \textbf{0.30} & 5.00* & \textbf{0.27} \\ 

Healthcare1 & 30.00* & \textbf{0.48} & 30.00 & - & 30.00 & - & 30.00* & \textbf{0.39} & 30.00* & \textbf{0.38} \\ 

Healthcare2 & 14.00 & \textbf{0.95} & 16.00 & - & 14.00 & \textbf{1.10} & 14.00 & \textbf{0.85} & 14.00 & \textbf{0.91} \\ 

Healthcare3 & 34.00* & \textbf{2.57} & 34.00* & \textbf{2.68} & 34.00* & \textbf{3.33} & 34.00* & \textbf{2.65} & 34.00* & \textbf{2.49} \\ 

Healthcare4 & 46.00* & \textbf{9.79} & 46.00* & \textbf{10.06} & 46.00* & \textbf{8.33} & 46.00* & \textbf{9.20} & 46.00* & \textbf{8.72} \\ 

Insurance & 527.00* & \textbf{25.53} & 527.00 & - & 527.00 & - & 527.00* & \textbf{23.13} & 527.00* & \textbf{24.21} \\ 

NetworkMgmt & 110.00* & \textbf{7.25} & 110.00* & \textbf{5.37} & 110.00* & \textbf{6.92} & 110.00* & \textbf{7.21} & 110.00* & \textbf{6.92} \\ 

ProcessorComm1 & 21.00 & \textbf{11.33} & 29.00 & - & 21.00 & \textbf{12.05} & 21.00 & \textbf{8.61} & 21.00 & \textbf{9.56} \\ 

ProcessorComm2 & 25.00* & \textbf{2.16} & 25.00* & \textbf{3.66} & 25.00* & \textbf{3.95} & 25.00* & \textbf{3.09} & 25.00* & \textbf{2.88} \\ 

Services & 100.00* & \textbf{12.46} & 100.00* & \textbf{6.52} & 100.00* & \textbf{12.43} & 100.00* & 16.64 & 100.00* & 14.21 \\ 

Storage1 & 17.00* & \textbf{0.41} & 17.00* & \textbf{0.31} & 17.00* & \textbf{0.37} & 17.00* & \textbf{0.31} & 17.00* & \textbf{0.30} \\ 

Storage2 & 18.00* & \textbf{0.45} & 18.00 & - & 18.00 & - & 18.00* & \textbf{0.34} & 18.00* & \textbf{0.30} \\ 

Storage3 & 50.00* & \textbf{2.38} & 50.00* & \textbf{2.96} & 50.00* & \textbf{2.99} & 50.00* & \textbf{2.21} & 50.00* & \textbf{3.56} \\ 

Storage4 & 130.00* & \textbf{6.84} & 130.00* & \textbf{6.75} & 130.00* & \textbf{7.79} & 130.00* & \textbf{6.69} & 130.00* & \textbf{6.95} \\ 

Storage5 & 215.00 & 247.99 & 218.00 & - & 215.00 & 339.78 & 215.00 & \textbf{214.04} & 218.00 & - \\ 

SystemMgmt & 15.00* & \textbf{0.49} & 15.00* & \textbf{0.36} & 15.00* & \textbf{0.43} & 15.00* & \textbf{0.36} & 15.00* & \textbf{0.35} \\ 

Telecom & 30.00* & \textbf{0.58} & 30.00* & \textbf{0.50} & 30.00* & \textbf{0.54} & 30.00* & \textbf{0.46} & 30.00* & \textbf{0.43} \\

\midrule %

Yu et al. \cite{Yu15} & & & & & & & & & & \\

\midrule

RL-A & 153.00 & \textbf{34.45} & 155.00 & - & 153.00 & 42.12 & 153.00 & \textbf{32.63} & 153.00 & \textbf{37.99} \\ 

RL-B & \textbf{745.80} & 5756.76 & 767.00 & - & 756.20 & - & 760.70 & 4888.94 & 767.00 & - \\ 

\midrule %

Yamada et al. \cite{Yamada16} & & & & & & & & & & \\

\midrule

Company2 & 72.00 & \textbf{3.28} & 81.00 & - & 72.00 & \textbf{4.74} & 72.00 & \textbf{4.79} & 72.00 & \textbf{3.46} \\

\bottomrule
\end{tabular}

}

\caption{Comparison of complete SAT-based MaxSAT approaches versus CALOT for the Covering Array Number problem.
Bold values represent the best results. In case of ties in size, the best time is marked. Times within a range of 1\% of the timeout (6.4 seconds) are considered as ties. For sizes with a star the optimum has been certified in at least one of the ten seeds executed.
}
\label{tab:ca}
\end{table}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/tables/table_ca_dom.tex <==
\begin{table}[h!t]
    \centering

    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{} & \multicolumn{2}{c|}{CALOT} & \multicolumn{2}{c|}{RC2-PM} & \multicolumn{2}{c|}{RC2-WPM} & \multicolumn{2}{c|}{Linear-PM} & \multicolumn{2}{c}{Linear-WPM} \\
         & size & time & size & time & size & time & size & time & size & time \\
        \midrule
        CALOT      & 0 0 &   0 0 &   \textbf{20} 0 &     \textbf{24} 4 &    \textbf{5} 4 &    \textbf{17} 8 &    5 5 &     \textbf{11} 8 &    4 \textbf{5} &     \textbf{11} 8 \\
        RC2-PM     & 0 \textbf{20} &  4 \textbf{24} &   0 0 &     0 0 &     0 \textbf{20} &   6 \textbf{20} &   0 \textbf{20} &     6 \textbf{24} &   0 \textbf{18} &     5 \textbf{23} \\
        RC2-WPM    & 4 \textbf{5} &   8 \textbf{17} &  \textbf{20} 0 &     \textbf{20} 6 &    0 0 &     0 0 &    \textbf{5} 4 &    9 \textbf{15} &    5 5 &     9 \textbf{14} \\
        Linear-PM  & 5 5 &   8 \textbf{11} &  \textbf{20} 0 &     \textbf{24} 6 &    4 \textbf{5} &    \textbf{15} 9 &    0 0 &     0 0 &    5 5 &     7 \textbf{8} \\
        Linear-WPM & \textbf{5} 4 &   8 \textbf{11} &  \textbf{18} 0 &     \textbf{23} 5 &    5 5 &     \textbf{14} 9 &    5 5 &     \textbf{8} 7 &    0 0 &     0 0 \\
        
        
        
        
        
        
        \bottomrule
    \end{tabular}
\caption{Dominance relations for CALOT and complete SAT-based MaxSAT approaches for the Covering Array Number problem.
Bold values highlight winning algorithm per size or runtime.
}
\label{tab:ca_dom}
\end{table}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/tables/table_ca_inc.tex <==
\begin{sidewaystable}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cr|cr|cr|cr|cr|cr|cr|cr|cr|cr|cr|cr}
\toprule
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{ACTS} & \multicolumn{2}{c|}{\makecell{CALOT \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{CALOT \\CCX a.1}} & \multicolumn{2}{c|}{\makecell{RC2-B \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{RC2-B \\CCX a.0 wpm}} & \multicolumn{2}{c|}{\makecell{linear \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{loandra \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{loandra \\CCX a.1}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.1}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.0 wpm}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.1 wpm}} \\
Instance & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time  \\
\midrule
Cohen et al. \cite{cohen2008constructing} \\
\midrule
1 & 48.00 & 0.83 & 38.00 & 1688.39 & 38.00 & 1470.88 & -1.00 & -1.00 & 37.00 & 7146.52 & 37.00 & 5367.02 & 37.00 & 1718.97 & \textbf{37.00} & \textbf{426.06} & 37.00 & 902.46 & 38.00 & 133.26 & 37.00 & 4724.61 & 38.00 & 1196.04 \\
2 & 32.00 & 1.08 & 30.00* & 2.80 & 30.00* & 3.57 & 30.00* & 9.85 & 30.00* & 10.81 & 30.00* & 2.91 & 30.00* & 7.19 & 30.00* & 7.68 & \textbf{30.00} & \textbf{0.81} & 30.00 & 1.42 & 30.00 & 0.92 & 30.00 & 1.70 \\
3 & 19.00 & 1.21 & 18.00* & 0.09 & 18.00* & 0.12 & 18.00* & 0.59 & 18.00* & 0.73 & 18.00* & 0.13 & 18.00* & 0.36 & 18.00* & 0.47 & 18.00 & 0.06 & 18.00 & 0.08 & \textbf{18.00} & \textbf{0.05} & 18.00 & 0.07 \\
4 & 22.00 & 1.04 & 20.00* & 0.52 & 20.00* & 0.95 & 20.00* & 2.58 & 20.00* & 3.19 & 20.00* & 0.74 & 20.00* & 1.34 & 20.00* & 2.24 & 20.00 & 0.30 & \textbf{20.00} & \textbf{0.29} & 20.00 & 0.31 & 20.00 & 0.45 \\
5 & 54.00 & 1.31 & 47.00 & 1955.92 & 48.00 & 241.15 & -1.00 & -1.00 & 48.00 & 378.46 & 47.00 & 1693.29 & 46.00 & 1629.29 & \textbf{\textbf{45.80}} & \textbf{1795.81} & 46.00 & 1624.87 & 46.00 & 1348.31 & 46.20 & 1803.99 & 46.00 & 4655.60 \\
6 & 25.00 & 1.11 & 24.00* & 1.18 & 24.00* & 1.46 & 24.00* & 4.46 & 24.00* & 5.47 & 24.00* & 1.48 & 24.00* & 2.98 & 24.00* & 3.51 & \textbf{24.00} & \textbf{0.33} & 24.00 & 0.48 & 24.00 & 0.34 & 24.00 & 0.47 \\
7 & 12.00 & 1.13 & 9.00 & 0.06 & 9.00 & 0.08 & -1.00 & -1.00 & 9.00 & 0.61 & 9.00 & 0.13 & 9.00 & 30.98 & 9.00 & 30.57 & 9.00 & 0.06 & 9.00 & 0.06 & \textbf{9.00} & \textbf{0.05} & 9.00 & 0.06 \\
8 & 47.00 & 1.01 & 38.00 & 1403.51 & 37.00 & 4727.41 & -1.00 & -1.00 & 37.00 & 3407.87 & 38.00 & 547.77 & 36.80* & 2849.90 & 37.00 & 3731.63 & 37.00 & 1178.58 & \textbf{\textbf{36.60}} & \textbf{2948.62} & 37.00 & 2333.83 & 37.00 & 5133.82 \\
9 & 22.00 & 1.21 & 20.00* & 0.57 & 20.00* & 0.84 & 20.00* & 2.36 & 20.00* & 2.66 & 20.00* & 0.49 & 20.00* & 1.22 & 20.00* & 2.30 & \textbf{20.00} & \textbf{0.18} & 20.00 & 0.27 & 20.00 & 0.19 & 20.00 & 0.41 \\
10 & 47.00 & 1.28 & 44.00 & 6860.63 & 44.20 & 5250.31 & -1.00 & -1.00 & 44.00 & 4759.95 & 44.00 & 1343.51 & 41.80 & 1235.36 & 41.00 & 1891.73 & 41.00 & 2720.18 & 41.00 & 970.10 & 41.00 & 5823.09 & \textbf{41.00} & \textbf{641.10} \\
11 & 47.00 & 1.26 & 41.00 & 2641.09 & 41.00 & 4167.69 & -1.00 & -1.00 & 42.00 & 6172.69 & 42.00 & 1916.85 & 39.00 & 6308.22 & 40.00 & 4323.47 & 40.00 & 741.96 & 40.00 & 1086.24 & \textbf{39.00} & \textbf{1628.02} & 39.00 & 2892.01 \\
12 & 43.00 & 1.29 & 36.00* & 14.13 & 36.00* & 24.01 & 36.00* & 36.81 & 36.00* & 49.94 & 36.00* & 20.66 & 36.00* & 36.16 & 36.00* & 42.45 & \textbf{36.00} & \textbf{8.18} & 36.00 & 10.46 & 36.00 & 10.75 & 36.00 & 11.37 \\
13 & 40.00 & 1.15 & 36.00* & 6.78 & 36.00* & 9.80 & 36.00* & 24.42 & 36.00* & 29.91 & 36.00* & 6.73 & 36.00* & 14.91 & 36.00* & 25.04 & 36.00 & 3.46 & 36.00 & 3.31 & \textbf{36.00} & \textbf{3.23} & 36.00 & 3.60 \\
14 & 39.00 & 0.83 & 36.00* & 3.76 & 36.00* & 5.25 & 36.00* & 13.81 & 36.00* & 15.56 & 36.00* & 4.80 & 36.00* & 8.84 & 36.00* & 11.51 & 36.00 & 1.89 & 36.00 & 2.48 & \textbf{36.00} & \textbf{1.51} & 36.00 & 4.28 \\
15 & 32.00 & 1.05 & 30.00* & 1.02 & 30.00* & 1.49 & 30.00* & 4.73 & 30.00* & 4.88 & 30.00* & 1.30 & 30.00* & 2.91 & 30.00* & 3.70 & \textbf{30.00} & \textbf{0.47} & 30.00 & 0.66 & 30.00 & 0.90 & 30.00 & 0.77 \\
16 & 25.00 & 0.84 & 24.00* & 1.36 & 24.00* & 1.94 & 24.00* & 5.59 & 24.00* & 6.60 & 24.00* & 1.65 & 24.00* & 4.30 & 24.00* & 4.46 & \textbf{24.00} & \textbf{0.56} & 24.00 & 0.60 & 24.00 & 0.57 & 24.00 & 0.62 \\
17 & 41.00 & 1.17 & 36.00* & 10.16 & 36.00* & 13.60 & 36.00* & 30.57 & 36.00* & 35.75 & 36.00* & 10.98 & 36.00* & 22.72 & 36.00* & 31.18 & \textbf{36.00} & \textbf{5.88} & 36.00 & 7.48 & 36.00 & 7.31 & 36.00 & 6.94 \\
18 & 52.00 & 1.30 & 42.00 & 128.65 & 42.00 & 201.42 & -1.00 & -1.00 & 42.00 & 177.28 & 42.00 & 202.10 & 41.00 & 637.62 & 41.00 & 734.99 & \textbf{41.00} & \textbf{134.63} & 41.00 & 626.83 & 41.00 & 2943.99 & 41.00 & 1871.62 \\
19 & 51.00 & 1.43 & 46.00 & 178.56 & 45.00 & 118.23 & -1.00 & -1.00 & 46.00 & 265.76 & 46.00 & 128.89 & 44.00 & 2056.11 & \textbf{\textbf{43.80}} & \textbf{2638.11} & 44.00 & 755.22 & 44.00 & 756.79 & 44.00 & 2892.85 & 44.00 & 578.78 \\
20 & 60.00 & 1.53 & 57.00 & 129.90 & 57.00 & 224.31 & -1.00 & -1.00 & 57.00 & 236.47 & 56.00 & 1092.85 & 54.80 & 1422.09 & \textbf{\textbf{54.60}} & \textbf{1736.92} & 55.00 & 32.47 & 55.00 & 500.42 & 55.00 & 437.94 & 55.00 & 176.33 \\
21 & 39.00 & 1.33 & 36.00* & 2.59 & 36.00* & 3.86 & 36.00* & 9.99 & 36.00* & 9.95 & 36.00* & 3.40 & 36.00* & 7.08 & 36.00* & 8.88 & \textbf{36.00} & \textbf{1.06} & 36.00 & 1.38 & 36.00 & 1.72 & 36.00 & 1.94 \\
22 & 37.00 & 1.08 & 36.00* & 1.75 & 36.00* & 2.70 & 36.00* & 7.74 & 36.00* & 8.57 & 36.00* & 2.17 & 36.00* & 5.25 & 36.00* & 6.78 & \textbf{36.00} & \textbf{0.65} & 36.00 & 0.88 & 36.00 & 0.72 & 36.00 & 1.04 \\
23 & 14.00 & 0.75 & 12.00* & 0.05 & 12.00* & 0.09 & 12.00* & 0.42 & 12.00* & 0.41 & 12.00* & 0.08 & 12.00* & 0.22 & 12.00* & 0.30 & \textbf{12.00} & \textbf{0.03} & 12.00 & 0.05 & 12.00 & 0.06 & 12.00 & 0.09 \\
24 & 48.00 & 1.40 & 44.40 & 4172.55 & 45.00 & 185.06 & -1.00 & -1.00 & 44.00 & 41.40 & 45.00 & 13.58 & 42.00 & 1693.19 & \textbf{\textbf{41.00}} & \textbf{4304.36} & 42.00 & 1465.17 & 43.00 & 59.40 & 42.00 & 884.17 & 42.00 & 926.51 \\
25 & 52.00 & 1.28 & 52.00 & 100.56 & 52.00 & 117.86 & -1.00 & -1.00 & -1.00 & -1.00 & 52.00 & 423.91 & 50.00 & 2069.85 & \textbf{\textbf{49.80}} & \textbf{1133.70} & 51.00 & 136.11 & 50.00 & 2101.71 & 50.00 & 5892.75 & 50.00 & 263.99 \\
26 & 34.00 & 1.37 & 27.00 & 49.99 & 27.00 & 31.54 & -1.00 & -1.00 & 27.00 & 112.13 & 27.00 & 551.57 & 27.00 & 103.46 & 27.00 & 57.66 & 26.00 & 6740.38 & \textbf{26.00} & \textbf{790.74} & 27.00 & 210.04 & 27.00 & 141.21 \\
27 & 37.00 & 1.32 & 36.00* & 1.14 & 36.00* & 1.68 & 36.00* & 5.35 & 36.00* & 6.70 & 36.00* & 1.33 & 36.00* & 2.96 & 36.00* & 3.56 & \textbf{36.00} & \textbf{0.39} & 36.00 & 0.61 & 36.00 & 0.45 & 36.00 & 0.62 \\
28 & 57.00 & 1.54 & 53.00 & 95.96 & 53.00 & 78.94 & -1.00 & -1.00 & 53.00 & 330.79 & 53.00 & 120.36 & 51.20 & 333.93 & 51.00 & 1236.07 & 51.00 & 3112.51 & 51.00 & 607.78 & 52.00 & 61.99 & \textbf{\textbf{49.00}} & \textbf{3329.73} \\
29 & 29.00 & 1.15 & 25.00* & 5.63 & 25.00* & 8.77 & 25.00* & 20.73 & 25.00* & 26.38 & 25.00* & 7.81 & 25.00* & 12.69 & 25.00* & 17.48 & \textbf{25.00} & \textbf{3.05} & 25.00 & 4.02 & 25.00 & 3.55 & 25.00 & 4.63 \\
30 & 22.00 & 0.81 & 16.00* & 1.38 & 16.00* & 1.75 & 16.00* & 4.53 & 16.00* & 5.98 & 16.00* & 1.56 & 16.00* & 3.57 & 16.00* & 3.94 & \textbf{16.00} & \textbf{0.68} & 16.00 & 0.83 & 16.00 & 0.77 & 16.00 & 1.08 \\
apache & 33.00 & 1.25 & 30.00* & 8.96 & 30.00* & 13.68 & 30.00* & 33.44 & 30.00* & 38.18 & 30.00* & 11.28 & 30.00* & 21.65 & 30.00* & 32.14 & \textbf{30.00} & \textbf{5.17} & 30.00 & 6.70 & 30.00 & 5.82 & 30.00 & 5.57 \\
bugzilla & 19.00 & 1.03 & 16.00* & 0.35 & 16.00* & 0.61 & 16.00* & 1.72 & 16.00* & 1.79 & 16.00* & 0.36 & 16.00* & 0.89 & 16.00* & 1.19 & \textbf{16.00} & \textbf{0.14} & 16.00 & 0.19 & 16.00 & 0.14 & 16.00 & 0.46 \\
gcc & 23.00 & 0.93 & 15.00 & 13.09 & 15.00 & 19.06 & -1.00 & -1.00 & 15.00 & 47.85 & 15.00 & 22.14 & 15.00 & 63.99 & 15.00 & 68.18 & \textbf{15.00} & \textbf{9.44} & 15.00 & 12.76 & 15.00 & 11.82 & 15.00 & 29.62 \\
spins & 26.00 & 1.22 & \textbf{19.00*} & \textbf{0.13} & 19.00* & 0.22 & 19.00* & 0.56 & 19.00* & 0.70 & 19.00* & 0.16 & 19.00* & 0.28 & 19.00* & 0.28 & 19.00 & 0.13 & 19.00 & 0.21 & 19.00 & 0.20 & 19.00 & 0.21 \\
spinv & 45.00 & 0.84 & 33.00 & 5.28 & 32.00 & 188.97 & -1.00 & -1.00 & 32.00 & 55.75 & 33.00 & 21.39 & 32.00 & 61.37 & 32.00 & 97.82 & \textbf{32.00} & \textbf{26.18} & 32.00 & 82.41 & 32.00 & 53.36 & 32.00 & 199.38 \\
\midrule
Segall et al. \cite{segall11} \\
\midrule
Banking1 & 15.00 & 0.85 & \textbf{13.00*} & \textbf{0.01} & 13.00* & 0.01 & 13.00* & 0.20 & 13.00* & 0.29 & 13.00* & 0.08 & 13.00* & 0.05 & 13.00* & 0.05 & 13.00 & 0.09 & 13.00 & 0.08 & 13.00 & 0.06 & 13.00 & 0.06 \\
Banking2 & 11.00 & 0.46 & \textbf{10.00*} & \textbf{0.01} & 10.00* & 0.02 & 10.00* & 25.56 & 10.00* & 22.95 & 10.00* & 0.03 & 10.00* & 19.30 & 10.00* & 10.62 & 10.00 & 0.02 & 10.00 & 0.02 & 10.00 & 0.02 & 10.00 & 0.02 \\
CommProtocol & 19.00 & 1.05 & \textbf{16.00*} & \textbf{0.02} & 16.00* & 0.03 & 16.00* & 0.19 & 16.00* & 0.22 & 16.00* & 0.03 & 16.00* & 0.15 & 16.00* & 0.09 & 16.00 & 0.05 & 16.00 & 0.03 & 16.00 & 0.02 & 16.00 & 0.02 \\
Concurrency & 6.00 & 0.49 & \textbf{5.00*} & \textbf{0.00} & 5.00* & 0.00 & 5.00* & 0.08 & 5.00* & 0.08 & 5.00* & 0.01 & 5.00* & 0.03 & 5.00* & 0.03 & 5.00 & 0.03 & 5.00 & 0.01 & 5.00 & 0.01 & 5.00 & 0.01 \\
Healthcare1 & 30.00 & 0.55 & 30.00* & 0.03 & 30.00* & 0.03 & 30.00* & 0.24 & 30.00* & 0.25 & 30.00* & 0.05 & 30.00* & 0.13 & 30.00* & 0.15 & 30.00 & 0.17 & 30.00 & 0.03 & \textbf{30.00} & \textbf{0.02} & 30.00 & 0.03 \\
Healthcare2 & 16.00 & 0.60 & \textbf{14.00} & \textbf{0.02} & 14.00 & 0.07 & -1.00 & -1.00 & 14.00 & 0.21 & 14.00 & 0.07 & 14.00 & 30.55 & 14.00 & 30.06 & 14.00 & 0.21 & 14.00 & 0.33 & 14.00 & 0.05 & 14.00 & 0.35 \\
Healthcare3 & 38.00 & 0.58 & 34.00* & 0.48 & 34.00* & 0.75 & 34.00* & 2.14 & 34.00* & 2.39 & 34.00* & 0.68 & 34.00* & 1.63 & 34.00* & 1.44 & \textbf{34.00} & \textbf{0.26} & 34.00 & 0.32 & 34.00 & 0.37 & 34.00 & 0.45 \\
Healthcare4 & 49.00 & 0.59 & 46.00* & 1.77 & 46.00* & 2.33 & 46.00* & 5.88 & 46.00* & 7.24 & 46.00* & 2.61 & 46.00* & 3.64 & 46.00* & 3.71 & \textbf{46.00} & \textbf{0.73} & 46.00 & 0.82 & 46.00 & 1.83 & 46.00 & 2.22 \\
Insurance & \textbf{527.00} & \textbf{0.31} & 527.00* & 16.82 & 527.00* & 18.56 & 527.00* & 44.42 & 527.00* & 45.47 & 527.00* & 21.08 & 527.00* & 45.23 & 527.00* & 46.40 & 527.00 & 5.29 & 527.00 & 10.47 & 527.00 & 5.08 & 527.00 & 11.25 \\
NetworkMgmt & 112.00 & 0.58 & 110.00* & 214.18 & 110.00* & 511.52 & 110.00* & 180.82 & 110.00* & 233.46 & 110.00* & 1100.79 & 110.00* & 45.65 & \textbf{110.00*} & \textbf{34.19} & 110.00 & 344.68 & 110.00 & 302.44 & 110.00 & 408.88 & 110.00 & 276.77 \\
ProcessorComm1 & 29.00 & 0.52 & 21.00 & 67.53 & 22.00 & 0.47 & -1.00 & -1.00 & 22.00 & 1.14 & \textbf{21.00} & \textbf{28.65} & 21.00 & 468.17 & 21.00 & 107.68 & 21.00 & 610.20 & 21.00 & 1690.90 & 22.00 & 0.22 & 21.00 & 1015.43 \\
ProcessorComm2 & 32.00 & 0.77 & 25.00* & 0.42 & 25.00* & 0.55 & 25.00* & 1.42 & 25.00* & 1.70 & 25.00* & 0.42 & 25.00* & 0.78 & 25.00* & 1.22 & \textbf{25.00} & \textbf{0.23} & 25.00 & 0.39 & 25.00 & 0.26 & 25.00 & 0.41 \\
Services & 106.00 & 1.20 & 100.00* & 28.65 & 100.00* & 29.89 & 100.00* & 40.55 & 100.00* & 37.37 & 100.00* & 26.69 & 100.00* & 3.94 & 100.00* & 3.97 & 100.00 & 2.43 & 100.00 & 2.44 & 100.00 & 2.42 & \textbf{100.00} & \textbf{1.46} \\
Storage1 & 17.00 & 0.75 & \textbf{17.00*} & \textbf{0.00} & 17.00* & 0.01 & 17.00* & 0.11 & 17.00* & 0.11 & 17.00* & 0.01 & -1.00 & -1.00 & -1.00 & -1.00 & 17.00 & 0.01 & 17.00 & 0.01 & 17.00 & 0.01 & 17.00 & 0.01 \\
Storage2 & 18.00 & 0.25 & \textbf{18.00*} & \textbf{0.01} & 18.00* & 0.01 & 18.00* & 0.12 & 18.00* & 0.12 & 18.00* & 0.02 & 18.00* & 0.05 & 18.00* & 0.05 & 18.00 & 0.02 & 18.00 & 0.01 & 18.00 & 0.01 & 18.00 & 0.01 \\
Storage3 & 50.00 & 0.66 & 50.00* & 0.14 & 50.00* & 0.28 & 50.00* & 11.02 & 50.00* & 1.86 & 50.00* & 0.26 & -1.00 & -1.00 & -1.00 & -1.00 & 50.00 & 0.09 & 50.00 & 0.11 & \textbf{50.00} & \textbf{0.08} & 50.00 & 0.12 \\
Storage4 & 136.00 & 0.60 & 130.00* & 2.49 & 130.00* & 3.24 & 130.00* & 7.24 & 130.00* & 9.28 & 130.00* & 1.69 & 130.00* & 5.16 & 130.00* & 6.65 & \textbf{130.00} & \textbf{0.55} & 130.00 & 0.84 & 130.00 & 0.58 & 130.00 & 0.83 \\
Storage5 & 218.00 & 0.87 & 215.00 & 68.48 & 215.00 & 389.33 & -1.00 & -1.00 & 215.00 & 140.68 & 215.00 & 811.43 & 215.00 & 85.07 & 215.00 & 90.98 & 215.00 & 17.01 & \textbf{215.00} & \textbf{16.83} & 215.00 & 45.27 & 215.00 & 46.54 \\
SystemMgmt & 17.00 & 0.57 & \textbf{15.00*} & \textbf{0.01} & 15.00* & 0.03 & 15.00* & 0.16 & 15.00* & 0.18 & 15.00* & 0.02 & 15.00* & 0.08 & 15.00* & 0.09 & 15.00 & 0.02 & 15.00 & 0.02 & 15.00 & 0.02 & 15.00 & 0.02 \\
Telecom & 32.00 & 0.58 & 30.00* & 0.04 & 30.00* & 0.05 & 30.00* & 0.31 & 30.00* & 0.37 & 30.00* & 0.06 & 30.00* & 0.18 & 30.00* & 0.22 & 30.00 & 0.03 & 30.00 & 0.04 & \textbf{30.00} & \textbf{0.03} & 30.00 & 0.04 \\
\midrule
Yu et al. \cite{Yu15} \\
\midrule
RL-A & 155.00 & 2.88 & 153.00 & 14.02 & 153.00 & 25.95 & -1.00 & -1.00 & 153.00 & 28.52 & 153.00 & 18.89 & 153.00 & 58.49 & 153.00 & 63.11 & \textbf{153.00} & \textbf{3.25} & 153.00 & 3.77 & 153.00 & 12.04 & 153.00 & 15.40 \\
RL-B & 767.00 & 170.61 & 760.00 & 4471.65 & 763.00 & 5862.61 & -1.00 & -1.00 & -1.00 & -1.00 & 764.00 & 5633.81 & -1.00 & -1.00 & -1.00 & -1.00 & -1.00 & -1.00 & \textbf{727.00} & \textbf{966.65} & -1.00 & -1.00 & 727.00 & 5809.65 \\
\midrule
Yamada et al. \cite{Yamada16} \\
\midrule
Company2 & 81.00 & 9.37 & 72.00 & 1.80 & 72.00 & 1.88 & -1.00 & -1.00 & 72.00 & 3.33 & 72.00 & 2.48 & 72.00 & 32.15 & 72.00 & 32.96 & \textbf{72.00} & \textbf{0.68} & 72.00 & 0.75 & 72.00 & 0.99 & 72.00 & 1.29 \\
\midrule
\bottomrule
\end{tabular}
}
\caption{Comparison of SAT-based MaxSAT approaches versus CALOT for the Covering Array Number problem.
Bold values represent the best results. In case of ties in size, the best time is marked. For sizes with a star the optimum has been certified in at least one of the five seeds executed.
}
\label{tab:ca-res}
\end{sidewaystable}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/tables/table_ca_inc_dom.tex <==
\begin{table}[h!t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c|}{\makecell{CALOT \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{CALOT \\CCX a.1}} & \multicolumn{2}{c|}{\makecell{RC2-B \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{RC2-B \\CCX a.0 wpm}} & \multicolumn{2}{c|}{\makecell{linear \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{loandra \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{loandra \\CCX a.1}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.0}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.1}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.0 wpm}} & \multicolumn{2}{c|}{\makecell{tt-open-wbo-inc \\CCX a.1 wpm}} \\
 & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time & size & time  \\
\midrule
ACTS & 0 \textbf{52} & 2 \textbf{56} & 0 \textbf{52} & 2 \textbf{56} & 21 \textbf{32} & 23 \textbf{35} & 2 \textbf{51} & 4 \textbf{54} & 0 \textbf{52} & 2 \textbf{56} & 3 \textbf{52} & 4 \textbf{54} & 3 \textbf{52} & 4 \textbf{54} & 1 \textbf{52} & 2 \textbf{56} & 0 \textbf{53} & 1 \textbf{57} & 1 \textbf{52} & 2 \textbf{56} & 0 \textbf{53} & 1 \textbf{57} \\
CALOT CCX a.0 & - - & - - & \textbf{5} 3 & \textbf{52} 6 & \textbf{21} 0 & \textbf{57} 1 & \textbf{5} 4 & \textbf{53} 5 & \textbf{3} 2 & \textbf{47} 11 & 3 \textbf{12} & \textbf{44} 14 & 3 \textbf{12} & \textbf{44} 14 & 1 \textbf{13} & 13 \textbf{45} & 0 \textbf{13} & 12 \textbf{46} & 2 \textbf{12} & 15 \textbf{43} & 0 \textbf{12} & 19 \textbf{39} \\
CALOT CCX a.1 & - - & - - & - - & - - & \textbf{21} 0 & \textbf{57} 1 & \textbf{4} 3 & \textbf{50} 8 & 5 \textbf{5} & 27 \textbf{31} & 3 \textbf{12} & \textbf{42} 16 & 3 \textbf{11} & \textbf{42} 16 & 1 \textbf{12} & 9 \textbf{49} & 0 \textbf{13} & 6 \textbf{52} & 1 \textbf{10} & 7 \textbf{51} & 0 \textbf{11} & 11 \textbf{47} \\
RC2-B CCX a.0 & - - & - - & - - & - - & - - & - - & 0 \textbf{19} & \textbf{31} 25 & 0 \textbf{21} & 1 \textbf{57} & 2 \textbf{20} & 3 \textbf{54} & 2 \textbf{20} & 6 \textbf{51} & 0 \textbf{20} & 1 \textbf{56} & 0 \textbf{21} & 1 \textbf{57} & 0 \textbf{20} & 1 \textbf{56} & 0 \textbf{21} & 1 \textbf{57} \\
RC2-B CCX a.0 wpm & - - & - - & - - & - - & - - & - - & - - & - - & 3 \textbf{5} & 7 \textbf{51} & 2 \textbf{11} & 8 \textbf{49} & 2 \textbf{10} & 10 \textbf{47} & 0 \textbf{11} & 1 \textbf{56} & 1 \textbf{13} & 4 \textbf{54} & 0 \textbf{9} & 2 \textbf{55} & 1 \textbf{11} & 6 \textbf{52} \\
linear CCX a.0 & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & 3 \textbf{11} & \textbf{41} 17 & 3 \textbf{11} & \textbf{41} 17 & 1 \textbf{12} & 7 \textbf{51} & 1 \textbf{13} & 4 \textbf{54} & 2 \textbf{11} & 3 \textbf{55} & 1 \textbf{12} & 7 \textbf{51} \\
loandra CCX a.0 & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & 2 \textbf{7} & \textbf{38} 17 & 4 \textbf{5} & 9 \textbf{48} & 4 \textbf{7} & 9 \textbf{49} & \textbf{5} 3 & 12 \textbf{45} & 3 \textbf{5} & 10 \textbf{48} \\
loandra CCX a.1 & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & \textbf{5} 3 & 13 \textbf{44} & \textbf{6} 5 & 9 \textbf{49} & \textbf{7} 3 & 13 \textbf{44} & \textbf{6} 5 & 13 \textbf{45} \\
tt-open-wbo-inc CCX a.0 & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & 2 \textbf{3} & \textbf{39} 19 & \textbf{4} 2 & \textbf{38} 19 & 2 \textbf{4} & \textbf{42} 16 \\
tt-open-wbo-inc CCX a.1 & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & \textbf{6} 3 & 21 \textbf{37} & 2 \textbf{3} & \textbf{39} 19 \\
tt-open-wbo-inc CCX a.0 wpm & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & - - & 1 \textbf{4} & \textbf{43} 15 \\
\bottomrule
\end{tabular}
}
\caption{Dominance relations for CALOT and SAT-based MaxSAT approaches for the Covering Array Number problem.
Bold values highlight winning algorithm per size or runtime.
}
\label{tab:ca-dom}
\end{table}

==> Incomplete MaxSAT Approaches for Combinatorial Testing (arXiv)/wpm1.tex <==
\newcommand{\graybox}[1]{%
  \begingroup
  \setlength{\fboxsep}{0pt}%
  \colorbox{gray!20}{\raisebox{0pt}[8pt][3pt]{#1}}%
  \endgroup
}

\begin{algorithm}[ht]
    \SetAlgoRefName{WPM1}
    \caption{Stratified WPM1}
    \label{alg:wpm1}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwInput}{Input:}
    \SetKw{KwAnd}{and}
    \SetKwProg{KwFunc}{function}{}{}
    \DontPrintSemicolon
    
    
    \KwInput{Weighted Partial MaxSAT formula $\phi$, SAT solver $sat$}
    
    
    
    $\phi_{wk}, \phi_{re}, status \leftarrow \emptyset, \phi, SAT$
    
    \While{True} {
        \If{status = SAT}{
            $sat.add(\phi_{st} \leftarrow$ next\_stratum$(\phi_{wk}, \phi_{re}))$
        
            $\phi_{wk}, \phi_{re} \leftarrow \phi_{wk} \cup \phi_{st}, \phi_{re} \setminus \phi_{st}$
        }
        
        \If{$(status \leftarrow sat.solve())=\mbox{SAT}$}{
            \lIf{$\phi_{re} = \emptyset$}{\Return{$(cost(sat.model, \phi), sat.model)$}}
        }
        
        \Else{
            
            \lIf{$(to\_relax \leftarrow \mbox{core\_analysis}(\phi_{wk}, sat.core))=\emptyset$} {\Return{$(\infty, \emptyset)$}}
        
            $relaxed, B\mbox{\graybox{, $residuals$}}  \leftarrow$ \graybox{split\_and\_}relax$(to\_relax, sat.n\_vars)$
            
            $sat.retract(to\_relax)$
            
            
            $sat.add(\phi_{rx} \leftarrow relaxed \cup (CNF(\sum_{b \in B} b = 1), \infty))$
            
            
            $\phi_{wk}, \phi_{re} \leftarrow (\phi_{wk} \setminus to\_relax) \cup \phi_{rx}, \phi_{re} \mbox{\graybox{$\cup \  residuals$}}$
            
            
            
        }
    }

\end{algorithm}


    
    
    
    
        
        
    
        
            
        
            
            



==> algo_incremental.tex <==
\newcommand{\satcomm}[1]{\textsf{\scriptsize #1}}
\begin{algorithm}[ht]
    \SetAlgoRefName{MSIncrementalCA}
    \caption{Incremental MaxSAT for Covering Array Construction \label{alg:incrmentalMS}}
    \SetKw{KwIfT}{?}
    \SetKw{KwElseT}{:}
    \SetKw{KwGoTo}{go to}
    \SetKwProg{KwFunc}{function}{}{}
    \SetKw{KwInput}{Input:}
    \SetKwComment{KwComm}{\#}{}
    \DontPrintSemicolon
    
    \KwInput{SUT model $S$, Tests $N_i$ per iteration, SAT-based MaxSAT solver $msat$}

    
    $T \leftarrow T \setminus ForbiddenTuples(S, msat)$ \KwComm{\satcomm{See Algorithm~\ref{ForbiddenAlg}}}
    
    $\phi_h, \phi_s \leftarrow PMSat_{CCX}^{N_i,t,S,lb}$
    
    $msat.add(\phi_h)$
    
    $msat.add\_retractable(\phi_s)$
    
    \While {$T \neq \emptyset$}{
    
    
        $msat.solve()$\; %
    
        $\gamma \leftarrow msat.model$\; 
        
        $\Gamma \leftarrow \Gamma \cup \gamma$\;
        
        Remove from $T$ the tuples covered by $\gamma$\;
        
        \hl{ TODO }
    }
\end{algorithm}
\let\satcomm\undefined

==> plots/plot_shortening_test_cmp.tex <==
\begin{figure}[h!t]
    \caption{Comparison of the required number of tests for different methods to cover as much tuples at each test from $\simeq T(N,t,S)$ (as base). %
    }
    \label{fig:hybrid-test-diff}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_1.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_11.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_20.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_benchmark_spinv.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_NetworkMgmt.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_Storage5.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_RL-A-mod.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tuples_Fig4/Gtuples_RL-B-mod.pdf}
\end{figure}

==> plots/plot_shortening_tuple_cmp.tex <==
\begin{figure}[h!t]
    \caption{Comparison of the required number of tests for different methods with regards to the number of test used by $\simeq T(N,t,S)$ (as base) to cover each number of tuples. %
    }
    \label{fig:hybrid-tests}
    \centering
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_1.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_11.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_20.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_benchmark_spinv.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_NetworkMgmt.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_Storage5.pdf} \\
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_RL-A-mod.pdf}
    \includegraphics[width=0.4\textwidth]{plots/shortening_comparison/tests_Fig3/Gtests_RL-B-mod.pdf}
\end{figure}

==> plots/shoretning_loandra_sat4j_cmp.tex <==
\begin{figure}[h!t]
    \caption{Number of additional tuples covered by \emph{loandra} respect to \emph{linear} approach for different test suite sizes.}
    \label{fig:shortening-cmp}
    \centering
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_1.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_11.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_20.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/benchmark_spinv.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/NetworkMgmt.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/Storage5.pdf} \\
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/RL-A-mod.pdf}
    \includegraphics[width=0.41\textwidth]{plots/shortening_loandra_sat4j_cmp/RL-B-mod.pdf}

\end{figure}

==> table-maxsat-comp.tex <==
\begin{table}[h!]
\caption{COMPARISON WITH EXISTING SAT-BASED APPROACHES FOR 2-WAY COVERAGE}
\centering

\begin{tabular}{lll|cc|cc|cc|cc|cc}

\multicolumn{3}{c}{\textbf{}} & \multicolumn{2}{|c}{rc2-PM-2} & \multicolumn{2}{|c}{rc2-WPM-2} & \multicolumn{2}{|c}{algorithm2} & \multicolumn{2}{|c}{sat4j-PM-2} & \multicolumn{2}{|c}{sat4j-WPM-2} \\
Name & Model & Constraints & size & time & size & time & size & time & size & time & size & time \\
\midrule

1 & $2^{86}3^{3}4^{1}5^{5}6^{2}$ & $2^{20}3^{3}4^{1}$ & 48.00 & -1.00 & 38.00 & 3996.66 & 36.60* & 2652.88 & 36.50* & 2308.89 & 36.80* & \textbf{1649.59} \\ 

10 & $2^{130}3^{6}4^{5}5^{2}6^{4}$ & $2^{40}3^{7}$ & 47.00 & -1.00 & 43.00 & 4902.71 & \textbf{38.07} & 2443.95 & 38.10 & 2827.92 & 38.20 & 2162.16 \\ 

11 & $2^{84}3^{4}4^{2}5^{2}6^{4}$ & $2^{28}3^{4}$ & 47.00 & -1.00 & 41.00 & 3433.48 & 38.07 & 1855.12 & 38.00 & 1935.20 & \textbf{37.80} & 3169.15 \\ 

12 & $2^{136}3^{4}4^{3}5^{1}6^{3}$ & $2^{23}3^{4}$ & 36.00* & \textbf{43.63} & 36.00* & 44.33 & 36.00* & 121.76 & 36.00* & 178.08 & 36.00* & 158.01 \\ 

13 & $2^{124}3^{4}4^{1}5^{2}6^{2}$ & $2^{22}3^{4}$ & 36.00* & \textbf{24.47} & 36.00* & 25.02 & 36.00* & 81.66 & 36.00* & 79.84 & 36.00* & 28.48 \\ 

14 & $2^{81}3^{5}4^{3}6^{3}$ & $2^{13}3^{2}$ & 36.00* & \textbf{13.32} & 36.00* & 13.65 & 36.00* & 34.75 & 36.00* & 36.31 & 36.00* & 14.57 \\ 

15 & $2^{50}3^{4}4^{1}5^{2}6^{1}$ & $2^{20}3^{2}$ & 30.00* & 4.50 & 30.00* & 4.54 & 30.00* & 4.01 & 30.00* & 3.83 & 30.00* & \textbf{3.82} \\ 

16 & $2^{81}3^{3}4^{2}6^{1}$ & $2^{30}3^{4}$ & 24.00* & 6.09 & 24.00* & 6.05 & 24.00* & \textbf{5.55} & 24.00* & 5.78 & 24.00* & 5.77 \\ 

17 & $2^{128}3^{3}4^{2}5^{1}6^{3}$ & $2^{25}3^{4}$ & 36.00* & 30.30 & 36.00* & \textbf{29.76} & 36.00* & 110.03 & 36.00* & 109.52 & 36.00* & 115.03 \\ 

18 & $2^{127}3^{2}4^{4}5^{6}6^{2}$ & $2^{23}3^{4}4^{1}$ & 52.00 & -1.00 & 42.00 & 76.28 & 39.60 & 1674.05 & 39.50 & 3051.03 & \textbf{39.40} & 3579.32 \\ 

19 & $2^{172}3^{9}4^{9}5^{3}6^{4}$ & $2^{38}3^{5}$ & 51.00 & -1.00 & 46.00 & 109.47 & \textbf{40.47} & 3682.16 & 40.90 & 3627.69 & 40.60 & 2942.67 \\ 

2 & $2^{86}3^{3}4^{3}5^{1}6^{1}$ & $2^{19}3^{3}$ & 30.00* & 10.08 & 30.00* & 10.26 & 30.00* & 10.13 & 30.00* & 10.14 & 30.00* & \textbf{9.99} \\ 

20 & $2^{138}3^{4}4^{5}5^{4}6^{7}$ & $2^{42}3^{6}$ & 60.00 & -1.00 & 56.00 & 480.64 & 52.80 & 3412.95 & 52.70 & 3527.27 & \textbf{52.60} & 3134.99 \\ 

21 & $2^{76}3^{3}4^{2}5^{1}6^{3}$ & $2^{40}3^{6}$ & 36.00* & \textbf{9.89} & 36.00* & 10.06 & 36.00* & 10.17 & 36.00* & 10.63 & 36.00* & 10.37 \\ 

22 & $2^{72}3^{4}4^{1}6^{2}$ & $2^{20}3^{2}$ & 36.00* & 7.68 & 36.00* & 7.79 & 36.00* & 6.71 & 36.00* & \textbf{6.25} & 36.00* & 6.25 \\ 

23 & $2^{25}3^{1}6^{1}$ & $2^{13}3^{2}$ & 12.00* & 0.75 & 12.00* & 0.75 & 12.00* & 0.72 & 12.00* & 0.66 & 12.00* & \textbf{0.65} \\ 

24 & $2^{110}3^{2}5^{3}6^{4}$ & $2^{25}3^{4}$ & 48.00 & -1.00 & 44.00 & 448.46 & \textbf{40.13} & 1910.20 & 40.20 & 2058.91 & 40.20 & 2852.32 \\ 

25 & $2^{118}3^{6}4^{2}5^{2}6^{6}$ & $2^{23}3^{3}4^{1}$ & 52.00 & -1.00 & 52.00 & -1.00 & \textbf{47.33} & 3057.30 & 47.60 & 3032.79 & 47.80 & 2274.16 \\ 

26 & $2^{87}3^{1}4^{3}5^{4}$ & $2^{28}3^{4}$ & 34.00 & -1.00 & 27.00 & \textbf{110.50} & 26.00 & 328.98 & 26.00 & 281.25 & 26.00 & 210.68 \\ 

27 & $2^{55}3^{2}4^{2}5^{1}6^{2}$ & $2^{17}3^{3}$ & 36.00* & 5.56 & 36.00* & 5.64 & 36.00* & 4.35 & 36.00* & 4.33 & 36.00* & \textbf{4.30} \\ 

28 & $2^{167}3^{16}4^{2}5^{3}6^{6}$ & $2^{31}3^{6}$ & 57.00 & -1.00 & 53.00 & \textbf{304.47} & 48.60 & 4026.57 & 48.60 & 4637.53 & 48.60 & 4431.50 \\ 

29 & $2^{134}3^{7}5^{3}$ & $2^{19}3^{3}$ & 25.00* & \textbf{20.95} & 25.00* & 21.79 & 25.00* & 24.24 & 25.00* & 29.05 & 25.00* & 30.16 \\ 

3 & $2^{27}4^{2}$ & $2^{9}3^{1}$ & 17.58* & 0.92 & 18.00* & 0.92 & 18.00* & 0.87 & 18.00* & \textbf{0.79} & 18.00* & 0.80 \\ 

30 & $2^{73}3^{3}4^{3}$ & $2^{31}3^{4}$ & 16.00* & 4.98 & 16.00* & 5.32 & 16.00* & \textbf{4.88} & 16.00* & 5.22 & 16.00* & 5.30 \\ 

4 & $2^{51}3^{4}4^{2}5^{1}$ & $2^{15}3^{2}$ & 20.00* & 3.01 & 20.00* & 3.03 & 20.00* & \textbf{2.41} & 20.00* & 2.43 & 20.00* & 2.46 \\ 

5 & $2^{155}3^{7}4^{3}5^{5}6^{4}$ & $2^{32}3^{6}4^{1}$ & 54.00 & -1.00 & 47.00 & 385.93 & \textbf{44.67} & 3140.94 & 44.80 & 2719.70 & 44.80 & 2213.57 \\ 

6 & $2^{73}4^{3}6^{1}$ & $2^{26}3^{4}$ & 24.00* & 4.83 & 24.00* & 4.82 & 24.00* & 4.55 & 24.00* & \textbf{4.38} & 24.00* & 4.45 \\ 

7 & $2^{29}3^{1}$ & $2^{13}3^{2}$ & 12.00 & -1.00 & 9.00 & 1.35 & 9.00 & 1.34 & 9.00 & 1.09 & 9.00 & \textbf{1.08} \\ 

8 & $2^{109}3^{2}4^{2}5^{3}6^{3}$ & $2^{32}3^{4}4^{1}$ & 47.00 & -1.00 & 38.00 & \textbf{340.90} & 36.00* & 1347.87 & 36.00* & 1085.48 & 36.00* & 992.90 \\ 

9 & $2^{57}3^{1}4^{1}5^{1}6^{1}$ & $2^{30}3^{7}$ & 20.00* & 2.80 & 20.00* & 2.85 & 20.00* & \textbf{2.20} & 20.00* & 2.25 & 20.00* & 2.24 \\ 

apache & $2^{158}3^{8}4^{4}5^{1}6^{1}$ & $2^{3}3^{1}4^{2}5^{1}$ & 30.00* & \textbf{33.58} & 30.00* & 35.32 & 30.00* & 111.19 & 30.00* & 105.05 & 30.00* & 110.21 \\ 

bugzilla & $2^{49}3^{1}4^{2}$ & $2^{4}3^{1}$ & 16.00* & 2.10 & 16.00* & 2.14 & 16.00* & \textbf{1.97} & 16.00* & 2.04 & 16.00* & 2.02 \\ 

gcc & $2^{189}3^{10}$ & $2^{37}3^{3}$ & 23.00 & -1.00 & 15.00 & \textbf{39.49} & 15.00 & 158.53 & 15.00 & 225.79 & 15.00 & 259.00 \\ 

spins & $2^{13}4^{5}$ & $2^{13}$ & 18.00* & \textbf{0.86} & 19.00* & 0.94 & 19.00* & 1.06 & 19.00* & 0.93 & 19.00* & 1.65 \\ 

spinv & $2^{42}3^{2}4^{11}$ & $2^{47}3^{2}$ & 45.00 & -1.00 & 32.00 & 134.94 & 31.00 & 115.57 & 31.00 & 153.66 & 31.00 & \textbf{90.75} \\ 

\end{tabular}

\end{table}

==> tables/table_ca.tex <==
\begin{table}[h!t]

\centering

\resizebox{0.83\textwidth}{!}{

\begin{tabular}{l|cr|cr|cr|cr|cr}
\toprule
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{CALOT} & \multicolumn{2}{c|}{RC2-PM} & \multicolumn{2}{c|}{RC2-WPM} & \multicolumn{2}{c|}{Linear-PM} & \multicolumn{2}{c}{Linear-WPM} \\
Instance & size & time & size & time & size & time & size & time & size & time \\
\midrule %

Cohen et al. \cite{cohen2008constructing} & & & & & & & & & & \\

\midrule

1 & 36.60* & 2097.94 & 38.40* & - & 36.40* & 2746.61 & 36.40* & 2666.12 & 36.40* & \textbf{1767.29} \\ 

2 & 30.00* & \textbf{9.63} & 30.00* & \textbf{12.05} & 30.00* & \textbf{12.72} & 30.00* & \textbf{10.44} & 30.00* & \textbf{10.54} \\ 

3 & 18.00* & \textbf{0.79} & 18.00* & \textbf{0.97} & 18.00* & \textbf{0.99} & 18.00* & \textbf{0.78} & 18.00* & \textbf{0.78} \\ 

4 & 20.00* & \textbf{2.27} & 20.00* & \textbf{3.13} & 20.00* & \textbf{3.22} & 20.00* & \textbf{2.38} & 20.00* & \textbf{2.35} \\ 

5 & 44.60 & 3039.80 & 54.00 & - & 44.60 & 3004.00 & 44.70 & 2538.28 & \textbf{44.40} & 3098.15 \\ 

6 & 24.00* & \textbf{4.33} & 24.00* & \textbf{5.56} & 24.00* & \textbf{5.50} & 24.00* & \textbf{5.02} & 24.00* & \textbf{4.98} \\ 

7 & 9.00 & \textbf{1.00} & 12.00 & - & 9.00 & \textbf{1.63} & 9.00 & \textbf{1.27} & 9.00 & \textbf{1.21} \\ 

8 & 36.00* & 1024.22 & 36.00* & 1019.61 & 36.00* & 1221.64 & 36.00* & 1227.26 & 36.00* & \textbf{944.89} \\ 

9 & 20.00* & \textbf{2.15} & 20.00* & \textbf{2.91} & 20.00* & \textbf{2.92} & 20.00* & \textbf{2.30} & 20.00* & \textbf{2.28} \\ 

10 & 38.30 & 1960.09 & 47.00 & - & 38.20 & 2322.41 & \textbf{38.10} & 2901.29 & 38.50 & 1962.17 \\ 

11 & 37.90 & 2701.45 & 47.00 & - & 37.90 & 2305.90 & 37.80 & 2808.34 & \textbf{37.70} & 2799.72 \\ 

12 & 36.00* & \textbf{114.89} & 36.00* & \textbf{118.78} & 36.00* & 194.74 & 36.00* & 148.69 & 36.00* & 143.26 \\ 

13 & 36.00* & 78.88 & 36.00* & \textbf{31.70} & 36.00* & 93.00 & 36.00* & \textbf{34.63} & 36.00* & \textbf{33.34} \\ 

14 & 36.00* & 32.78 & 36.00* & \textbf{14.68} & 36.00* & \textbf{17.00} & 36.00* & 34.61 & 36.00* & 36.91 \\ 

15 & 30.00* & \textbf{3.85} & 30.00* & \textbf{4.77} & 30.00* & \textbf{4.86} & 30.00* & \textbf{3.68} & 30.00* & \textbf{3.61} \\ 

16 & 24.00* & \textbf{5.27} & 24.00* & \textbf{7.58} & 24.00* & \textbf{7.61} & 24.00* & \textbf{5.78} & 24.00* & \textbf{5.71} \\ 

17 & 36.00* & 99.88 & 36.00* & \textbf{65.09} & 36.00* & 125.62 & 36.00* & 104.08 & 36.00* & 112.25 \\ 

18 & 39.70 & 1825.61 & 52.00 & - & 39.30 & \textbf{2112.41} & 39.40 & 3560.15 & 39.30 & 3794.11 \\ 

19 & 40.50 & 3494.11 & 51.00 & - & 40.60 & 3627.53 & 40.80 & 3356.22 & \textbf{40.40} & 4150.12 \\ 

20 & 52.70 & 3719.47 & 60.00 & - & \textbf{52.50} & \textbf{3571.71} & 52.90 & 3743.61 & 52.70 & 4096.86 \\ 

21 & 36.00* & \textbf{9.73} & 36.00* & \textbf{11.63} & 36.00* & \textbf{12.00} & 36.00* & \textbf{9.73} & 36.00* & \textbf{9.83} \\ 

22 & 36.00* & \textbf{6.32} & 36.00* & \textbf{9.03} & 36.00* & \textbf{9.17} & 36.00* & \textbf{7.00} & 36.00* & \textbf{6.94} \\ 

23 & 12.00* & \textbf{0.65} & 12.00* & \textbf{0.74} & 12.00* & \textbf{0.74} & 12.00* & \textbf{0.60} & 12.00* & \textbf{0.60} \\ 

24 & 40.10 & \textbf{2322.47} & 48.00 & - & 40.60 & 1434.60 & 40.10 & 3233.78 & 40.10 & 2373.92 \\ 

25 & 47.30 & 3502.14 & 52.00 & - & 47.50 & 3792.21 & \textbf{47.10} & 3295.66 & 47.30 & 3135.00 \\ 

26 & 26.00 & 251.66 & 34.00 & - & 26.00 & \textbf{165.95} & 26.00 & 187.65 & 26.00 & 254.04 \\ 

27 & 36.00* & \textbf{4.08} & 36.00* & \textbf{6.20} & 36.00* & \textbf{6.21} & 36.00* & \textbf{4.39} & 36.00* & \textbf{4.33} \\ 

28 & \textbf{48.40} & 4034.09 & 57.00 & - & 48.50 & 4436.71 & 48.50 & 4082.97 & 48.60 & 3904.62 \\ 

29 & 25.00* & \textbf{22.93} & 25.00* & 58.71 & 25.00* & 65.48 & 25.00* & 32.20 & 25.00* & 29.63 \\ 

30 & 16.00* & \textbf{4.59} & 16.00* & \textbf{5.71} & 16.00* & \textbf{6.22} & 16.00* & \textbf{6.04} & 16.00* & \textbf{6.05} \\ 

apache & 30.00* & 106.62 & 30.00* & \textbf{93.83} & 30.00* & 117.45 & 30.00* & 124.21 & 30.00* & 118.02 \\ 

bugzilla & 16.00* & \textbf{1.84} & 16.00* & \textbf{2.36} & 16.00* & \textbf{2.39} & 16.00* & \textbf{1.97} & 16.00* & \textbf{1.95} \\ 

gcc & 15.00 & \textbf{149.50} & 23.00 & - & 15.00 & 187.58 & 15.00 & 253.12 & 15.00 & 250.03 \\ 

spins & 19.00* & \textbf{0.96} & 19.00* & \textbf{1.00} & 19.00* & \textbf{1.69} & 19.00* & \textbf{1.41} & 19.00* & \textbf{1.38} \\ 

spinv & 31.00 & \textbf{106.02} & 45.00 & - & 31.00 & \textbf{104.61} & 31.00 & \textbf{110.06} & 31.00 & \textbf{106.76} \\ 

\midrule %

Segall et al. \cite{segall11} & & & & & & & & & & \\

\midrule

Banking1 & 13.00* & \textbf{0.57} & 13.00* & \textbf{0.45} & 13.00* & \textbf{0.51} & 13.00* & \textbf{0.45} & 13.00* & \textbf{0.40} \\ 

Banking2 & 10.00* & \textbf{9.04} & 10.00* & \textbf{14.47} & 10.00* & \textbf{14.38} & 10.00* & \textbf{9.25} & 10.00* & \textbf{9.11} \\ 

CommProtocol & 16.00* & \textbf{0.50} & 16.00* & \textbf{0.40} & 16.00* & \textbf{0.46} & 16.00* & \textbf{0.39} & 16.00* & \textbf{0.35} \\ 

Concurrency & 5.00* & \textbf{0.40} & 5.00* & \textbf{0.28} & 5.00* & \textbf{0.32} & 5.00* & \textbf{0.30} & 5.00* & \textbf{0.27} \\ 

Healthcare1 & 30.00* & \textbf{0.48} & 30.00 & - & 30.00 & - & 30.00* & \textbf{0.39} & 30.00* & \textbf{0.38} \\ 

Healthcare2 & 14.00 & \textbf{0.95} & 16.00 & - & 14.00 & \textbf{1.10} & 14.00 & \textbf{0.85} & 14.00 & \textbf{0.91} \\ 

Healthcare3 & 34.00* & \textbf{2.57} & 34.00* & \textbf{2.68} & 34.00* & \textbf{3.33} & 34.00* & \textbf{2.65} & 34.00* & \textbf{2.49} \\ 

Healthcare4 & 46.00* & \textbf{9.79} & 46.00* & \textbf{10.06} & 46.00* & \textbf{8.33} & 46.00* & \textbf{9.20} & 46.00* & \textbf{8.72} \\ 

Insurance & 527.00* & \textbf{25.53} & 527.00 & - & 527.00 & - & 527.00* & \textbf{23.13} & 527.00* & \textbf{24.21} \\ 

NetworkMgmt & 110.00* & \textbf{7.25} & 110.00* & \textbf{5.37} & 110.00* & \textbf{6.92} & 110.00* & \textbf{7.21} & 110.00* & \textbf{6.92} \\ 

ProcessorComm1 & 21.00 & \textbf{11.33} & 29.00 & - & 21.00 & \textbf{12.05} & 21.00 & \textbf{8.61} & 21.00 & \textbf{9.56} \\ 

ProcessorComm2 & 25.00* & \textbf{2.16} & 25.00* & \textbf{3.66} & 25.00* & \textbf{3.95} & 25.00* & \textbf{3.09} & 25.00* & \textbf{2.88} \\ 

Services & 100.00* & \textbf{12.46} & 100.00* & \textbf{6.52} & 100.00* & \textbf{12.43} & 100.00* & 16.64 & 100.00* & 14.21 \\ 

Storage1 & 17.00* & \textbf{0.41} & 17.00* & \textbf{0.31} & 17.00* & \textbf{0.37} & 17.00* & \textbf{0.31} & 17.00* & \textbf{0.30} \\ 

Storage2 & 18.00* & \textbf{0.45} & 18.00 & - & 18.00 & - & 18.00* & \textbf{0.34} & 18.00* & \textbf{0.30} \\ 

Storage3 & 50.00* & \textbf{2.38} & 50.00* & \textbf{2.96} & 50.00* & \textbf{2.99} & 50.00* & \textbf{2.21} & 50.00* & \textbf{3.56} \\ 

Storage4 & 130.00* & \textbf{6.84} & 130.00* & \textbf{6.75} & 130.00* & \textbf{7.79} & 130.00* & \textbf{6.69} & 130.00* & \textbf{6.95} \\ 

Storage5 & 215.00 & 247.99 & 218.00 & - & 215.00 & 339.78 & 215.00 & \textbf{214.04} & 218.00 & - \\ 

SystemMgmt & 15.00* & \textbf{0.49} & 15.00* & \textbf{0.36} & 15.00* & \textbf{0.43} & 15.00* & \textbf{0.36} & 15.00* & \textbf{0.35} \\ 

Telecom & 30.00* & \textbf{0.58} & 30.00* & \textbf{0.50} & 30.00* & \textbf{0.54} & 30.00* & \textbf{0.46} & 30.00* & \textbf{0.43} \\

\midrule %

Yu et al. \cite{Yu15} & & & & & & & & & & \\

\midrule

RL-A & 153.00 & \textbf{34.45} & 155.00 & - & 153.00 & 42.12 & 153.00 & \textbf{32.63} & 153.00 & \textbf{37.99} \\ 

RL-B & \textbf{745.80} & 5756.76 & 767.00 & - & 756.20 & - & 760.70 & 4888.94 & 767.00 & - \\ 

\midrule %

Yamada et al. \cite{Yamada16} & & & & & & & & & & \\

\midrule

Company2 & 72.00 & \textbf{3.28} & 81.00 & - & 72.00 & \textbf{4.74} & 72.00 & \textbf{4.79} & 72.00 & \textbf{3.46} \\

\bottomrule
\end{tabular}

}

\caption{Comparison of complete SAT-based MaxSAT approaches versus CALOT for the Covering Array Number problem.
Bold values represent the best results. In case of ties in size, the best time is marked. Times within a range of 1\% of the timeout (6.4 seconds) are considered as ties. For sizes with a star the optimum has been certified in at least one of the ten seeds executed.
}
\label{tab:ca}
\end{table}

==> tables/table_ca_dom.tex <==
\begin{table}[h!t]
    \centering

    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{} & \multicolumn{2}{c|}{CALOT} & \multicolumn{2}{c|}{RC2-PM} & \multicolumn{2}{c|}{RC2-WPM} & \multicolumn{2}{c|}{Linear-PM} & \multicolumn{2}{c}{Linear-WPM} \\
         & size & time & size & time & size & time & size & time & size & time \\
        \midrule
        CALOT      & 0 0 &   0 0 &   \textbf{20} 0 &     \textbf{24} 4 &    \textbf{5} 4 &    \textbf{17} 8 &    5 5 &     \textbf{11} 8 &    4 \textbf{5} &     \textbf{11} 8 \\
        RC2-PM     & 0 \textbf{20} &  4 \textbf{24} &   0 0 &     0 0 &     0 \textbf{20} &   6 \textbf{20} &   0 \textbf{20} &     6 \textbf{24} &   0 \textbf{18} &     5 \textbf{23} \\
        RC2-WPM    & 4 \textbf{5} &   8 \textbf{17} &  \textbf{20} 0 &     \textbf{20} 6 &    0 0 &     0 0 &    \textbf{5} 4 &    9 \textbf{15} &    5 5 &     9 \textbf{14} \\
        Linear-PM  & 5 5 &   8 \textbf{11} &  \textbf{20} 0 &     \textbf{24} 6 &    4 \textbf{5} &    \textbf{15} 9 &    0 0 &     0 0 &    5 5 &     7 \textbf{8} \\
        Linear-WPM & \textbf{5} 4 &   8 \textbf{11} &  \textbf{18} 0 &     \textbf{23} 5 &    5 5 &     \textbf{14} 9 &    5 5 &     \textbf{8} 7 &    0 0 &     0 0 \\
        
        
        
        
        
        
        \bottomrule
    \end{tabular}
\caption{Dominance relations for CALOT and complete SAT-based MaxSAT approaches for the Covering Array Number problem.
Bold values highlight winning algorithm per size or runtime.
}
\label{tab:ca_dom}
\end{table}
